A Study on the Generality of Neural Network Structures for Monocular Depth Estimation

Monocular depth estimation has been widely studied, and significant improvements in performance have been recently reported. However, most previous works are evaluated on a few benchmark datasets, such as KITTI datasets, and none of the works provide an in-depth analysis of the generalization performance of monocular depth estimation. In this paper, we deeply investigate the various backbone networks (e.g.CNN and Transformer models) toward the generalization of monocular depth estimation. First, we evaluate state-of-the-art models on both in-distribution and out-of-distribution datasets, which have never been seen during network training. Then, we investigate the internal properties of the representations from the intermediate layers of CNN-/Transformer-based models using synthetic texture-shifted datasets. Through extensive experiments, we observe that the Transformers exhibit a strong shape-bias rather than CNNs, which have a strong texture-bias. We also discover that texture-biased models exhibit worse generalization performance for monocular depth estimation than shape-biased models. We demonstrate that similar aspects are observed in real-world driving datasets captured under diverse environments. Lastly, we conduct a dense ablation study with various backbone networks which are utilized in modern strategies. The experiments demonstrate that the intrinsic locality of the CNNs and the self-attention of the Transformers induce texture-bias and shape-bias, respectively.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> fig.tex <==
\begin{fig}

\begin{figure*}[t]
     \newcommand\w{10cm}
    \newcommand\h{5cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \includegraphics[width=\w,height=\h]{figure/sup_demon/img_mvs_0014.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/gt_mvs_0014.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/BTS_mvs_0014.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Adabins_mvs_0014.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Transdepth_mvs_0014.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Depthformer_mvs_0014.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/GLPDepth_mvs_0014.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/img_rgbd_0166.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/gt_rgbd_0166.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/BTS_rgbd_0166.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Adabins_rgbd_0166.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Transdepth_rgbd_0166.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Depthformer_rgbd_0166.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/GLPDepth_rgbd_0166.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/img_rgbd_0170.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/gt_rgbd_0170.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/BTS_rgbd_0170.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Adabins_rgbd_0170.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Transdepth_rgbd_0170.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Depthformer_rgbd_0170.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/GLPDepth_rgbd_0170.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/sup_demon/img_scenes11_0391.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/gt_scenes11_0391.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/BTS_scenes11_0391.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Adabins_scenes11_0391.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Transdepth_scenes11_0391.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Depthformer_scenes11_0391.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/GLPDepth_scenes11_0391.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/img_scenes11_0507.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/gt_scenes11_0507.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/BTS_scenes11_0507.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Adabins_scenes11_0507.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Transdepth_scenes11_0507.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Depthformer_scenes11_0507.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/GLPDepth_scenes11_0507.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/img_sun3d_0555.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/gt_sun3d_0555.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/BTS_sun3d_0555.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Adabins_sun3d_0555.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Transdepth_sun3d_0555.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/Depthformer_sun3d_0555.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/sup_demon/GLPDepth_sun3d_0555.pdf}\\ 

     \fontsize{40}{40} \selectfont Input images & 
     \fontsize{40}{40} \selectfont GT depths &
     \fontsize{40}{40} \selectfont BTS &
     \fontsize{40}{40} \selectfont AdaBins &
     \fontsize{40}{40} \selectfont TransDepth & 
     \fontsize{40}{40} \selectfont DepthFormer & 
     \fontsize{40}{40} \selectfont GLPDepth
    \end{tabular}}
    \caption{\textbf{Comparison of depth map results on various dataset.} We test our model and the competitive models trained on KITTI using MVS, SUN3D, RGBD, Scenes11 (Top to Bottom).}
    \label{figure_result_demons}
     \end{figure*}


\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccc}
     \includegraphics[]{figure/sup_kitti/img_KITTI_pencil_4.pdf}& 
     \includegraphics[]{figure/sup_kitti/KITTI_pencil_BTS_4.pdf}&  
     \includegraphics[]{figure/sup_kitti/KITTI_pencil_Adabins_4.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_pencil_Transdepth_4.pdf}&
      \includegraphics[]{figure/sup_kitti/KITTI_pencil_Depthformer_4.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_pencil_GLPDepth_4.pdf}\\
      \includegraphics[]{figure/sup_kitti/img_KITTI_pencil_9.pdf}& 
     \includegraphics[]{figure/sup_kitti/KITTI_pencil_BTS_9.pdf}&  
     \includegraphics[]{figure/sup_kitti/KITTI_pencil_Adabins_9.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_pencil_Transdepth_9.pdf}&
      \includegraphics[]{figure/sup_kitti/KITTI_pencil_Depthformer_9.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_pencil_GLPDepth_9.pdf}\\
          \includegraphics[]{figure/sup_kitti/img_KITTI_water_1.pdf}& 
     \includegraphics[]{figure/sup_kitti/KITTI_water_BTS_1.pdf}&  
     \includegraphics[]{figure/sup_kitti/KITTI_water_Adabins_1.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_water_Transdepth_1.pdf}&
      \includegraphics[]{figure/sup_kitti/KITTI_water_Depthformer_1.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_water_GLPDepth_1.pdf}\\
          \includegraphics[]{figure/sup_kitti/img_KITTI_water_13.pdf}& 
     \includegraphics[]{figure/sup_kitti/KITTI_water_BTS_13.pdf}&  
     \includegraphics[]{figure/sup_kitti/KITTI_water_Adabins_13.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_water_Transdepth_13.pdf}&
      \includegraphics[]{figure/sup_kitti/KITTI_water_Depthformer_13.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_water_GLPDepth_13.pdf}\\
          \includegraphics[]{figure/sup_kitti/img_KITTI_water_15.pdf}& 
     \includegraphics[]{figure/sup_kitti/KITTI_water_BTS_15.pdf}&  
     \includegraphics[]{figure/sup_kitti/KITTI_water_Adabins_15.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_water_Transdepth_15.pdf}&
      \includegraphics[]{figure/sup_kitti/KITTI_water_Depthformer_15.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_water_GLPDepth_15.pdf}\\
          \includegraphics[]{figure/sup_kitti/img_KITTI_style1_0.pdf}& 
     \includegraphics[]{figure/sup_kitti/KITTI_style1_BTS_0.pdf}&  
     \includegraphics[]{figure/sup_kitti/KITTI_style1_Adabins_0.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_style1_Transdepth_0.pdf}&
      \includegraphics[]{figure/sup_kitti/KITTI_style1_Depthformer_0.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_style1_GLPDepth_0.pdf}\\
          \includegraphics[]{figure/sup_kitti/img_KITTI_style1_3.pdf}& 
     \includegraphics[]{figure/sup_kitti/KITTI_style1_BTS_3.pdf}&  
     \includegraphics[]{figure/sup_kitti/KITTI_style1_Adabins_3.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_style1_Transdepth_3.pdf}&
      \includegraphics[]{figure/sup_kitti/KITTI_style1_Depthformer_3.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_style1_GLPDepth_3.pdf}\\
          \includegraphics[]{figure/sup_kitti/img_KITTI_style1_7.pdf}& 
     \includegraphics[]{figure/sup_kitti/KITTI_style1_BTS_7.pdf}&  
     \includegraphics[]{figure/sup_kitti/KITTI_style1_Adabins_7.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_style1_Transdepth_7.pdf}&
      \includegraphics[]{figure/sup_kitti/KITTI_style1_Depthformer_7.pdf}&
     \includegraphics[]{figure/sup_kitti/KITTI_style1_GLPDepth_7.pdf}\\
     
     \fontsize{120}{50} \selectfont Input images & \fontsize{120}{50} \selectfont BTS & 
     \fontsize{120}{50} \selectfont AdaBins&
     \fontsize{120}{50} \selectfont TransDepth& \fontsize{120}{50} \selectfont DepthFormer&
     \fontsize{120}{50} \selectfont GLPDepth
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\label{figure_result_kitti}
\end{figure*}

\begin{figure*}[t]
     \newcommand\w{10cm}
    \newcommand\h{5cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
        \includegraphics[width=\w,height=\h]{figure/sup_eth/img_courtyard_0000.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_courtyard_0000.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_courtyard_0000.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_courtyard_0000.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_courtyard_0000.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_courtyard_0000.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_courtyard_0000.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/sup_eth/img_courtyard_0013.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_courtyard_0013.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_courtyard_0013.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_courtyard_0013.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_courtyard_0013.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_courtyard_0013.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_courtyard_0013.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/sup_eth/img_delivery_area_0008.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_delivery_area_0008.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_delivery_area_0008.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_delivery_area_0008.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_delivery_area_0008.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_delivery_area_0008.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_delivery_area_0008.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/sup_eth/img_facade_0002.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_facade_0002.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_facade_0002.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_facade_0002.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_facade_0002.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_facade_0002.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_facade_0002.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/sup_eth/img_kicker_0008.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_kicker_0008.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_kicker_0008.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_kicker_0008.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_kicker_0008.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_kicker_0008.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_kicker_0008.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/sup_eth/img_kicker_0026.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_kicker_0026.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_kicker_0026.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_kicker_0026.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_kicker_0026.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_kicker_0026.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_kicker_0026.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/sup_eth/img_pipes_0004.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_pipes_0004.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_pipes_0004.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_pipes_0004.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_pipes_0004.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_pipes_0004.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_pipes_0004.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/sup_eth/img_pipes_0007.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_pipes_0007.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_pipes_0007.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_pipes_0007.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_pipes_0007.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_pipes_0007.pdf}&
        \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_pipes_0007.pdf}\\
     \fontsize{40}{40} \selectfont Input images & 
     \fontsize{40}{40} \selectfont GT depths &
     \fontsize{40}{40} \selectfont BTS &
     \fontsize{40}{40} \selectfont AdaBins &
     \fontsize{40}{40} \selectfont TransDepth & 
     \fontsize{40}{40} \selectfont DepthFormer & 
     \fontsize{40}{40} \selectfont GLPDepth
    \end{tabular}}
    \caption{\textbf{Comparison of depth map results on various dataset.} We test our model and the competitive models trained on KITTI using ETH3D (Top to Bottom).}
    \label{figure_result_demons}
     \end{figure*}

\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccc}
    \includegraphics[]{figure/selfsup_raincs/img_0.pdf}&
    \includegraphics[]{figure/selfsup_raincs/hybrid_0.pdf}&
    \includegraphics[]{figure/selfsup_raincs/vitb_0.pdf}&
    \includegraphics[]{figure/selfsup_raincs/monodepth2_0.pdf}&
    \includegraphics[]{figure/selfsup_raincs/packnet-sfm_0.pdf}&
    \includegraphics[]{figure/selfsup_raincs/rmsfm_0.pdf}\\
    \includegraphics[]{figure/selfsup_raincs/img_1.pdf}&
    \includegraphics[]{figure/selfsup_raincs/hybrid_1.pdf}&
    \includegraphics[]{figure/selfsup_raincs/vitb_1.pdf}&
    \includegraphics[]{figure/selfsup_raincs/monodepth2_1.pdf}&
    \includegraphics[]{figure/selfsup_raincs/packnet-sfm_1.pdf}&
    \includegraphics[]{figure/selfsup_raincs/rmsfm_1.pdf}\\
    \includegraphics[]{figure/selfsup_raincs/img_2.pdf}&
    \includegraphics[]{figure/selfsup_raincs/hybrid_2.pdf}&
    \includegraphics[]{figure/selfsup_raincs/vitb_2.pdf}&
    \includegraphics[]{figure/selfsup_raincs/monodepth2_2.pdf}&
    \includegraphics[]{figure/selfsup_raincs/packnet-sfm_2.pdf}&
    \includegraphics[]{figure/selfsup_raincs/rmsfm_2.pdf}\\
    \includegraphics[]{figure/selfsup_raincs/img_3.pdf}&
    \includegraphics[]{figure/selfsup_raincs/hybrid_3.pdf}&
    \includegraphics[]{figure/selfsup_raincs/vitb_3.pdf}&
    \includegraphics[]{figure/selfsup_raincs/monodepth2_3.pdf}&
    \includegraphics[]{figure/selfsup_raincs/packnet-sfm_3.pdf}&
    \includegraphics[]{figure/selfsup_raincs/rmsfm_3.pdf}\\
    \includegraphics[]{figure/selfsup_raincs/img_4.pdf}&
    \includegraphics[]{figure/selfsup_raincs/hybrid_4.pdf}&
    \includegraphics[]{figure/selfsup_raincs/vitb_4.pdf}&
    \includegraphics[]{figure/selfsup_raincs/monodepth2_4.pdf}&
    \includegraphics[]{figure/selfsup_raincs/packnet-sfm_4.pdf}&
    \includegraphics[]{figure/selfsup_raincs/rmsfm_4.pdf}\\
    \includegraphics[]{figure/selfsup_raincs/img_5.pdf}&
    \includegraphics[]{figure/selfsup_raincs/hybrid_5.pdf}&
    \includegraphics[]{figure/selfsup_raincs/vitb_5.pdf}&
    \includegraphics[]{figure/selfsup_raincs/monodepth2_5.pdf}&
    \includegraphics[]{figure/selfsup_raincs/packnet-sfm_5.pdf}&
    \includegraphics[]{figure/selfsup_raincs/rmsfm_5.pdf}\\
    \includegraphics[]{figure/selfsup_raincs/img_6.pdf}&
    \includegraphics[]{figure/selfsup_raincs/hybrid_6.pdf}&
    \includegraphics[]{figure/selfsup_raincs/vitb_6.pdf}&
    \includegraphics[]{figure/selfsup_raincs/monodepth2_6.pdf}&
    \includegraphics[]{figure/selfsup_raincs/packnet-sfm_6.pdf}&
    \includegraphics[]{figure/selfsup_raincs/rmsfm_6.pdf}\\
    \includegraphics[]{figure/selfsup_raincs/img_7.pdf}&
    \includegraphics[]{figure/selfsup_raincs/hybrid_7.pdf}&
    \includegraphics[]{figure/selfsup_raincs/vitb_7.pdf}&
    \includegraphics[]{figure/selfsup_raincs/monodepth2_7.pdf}&
    \includegraphics[]{figure/selfsup_raincs/packnet-sfm_7.pdf}&
    \includegraphics[]{figure/selfsup_raincs/rmsfm_7.pdf}\\
     \fontsize{120}{50} \selectfont Input images & \fontsize{120}{50} \selectfont Ours-Hybrid & 
     \fontsize{120}{50} \selectfont Ours-ViT&
     \fontsize{120}{50} \selectfont Monodepth2& \fontsize{120}{50} \selectfont PackNet-SfM&
     \fontsize{120}{50} \selectfont R-MSFM6
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\label{figure_result_kitti}
\end{figure*}

\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccc}
    \includegraphics[]{figure/selfsup_robotcar/img_0.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/hybrid_0.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/vitb_0.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/monodepth2_0.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/packnet-sfm_0.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/rmsfm_0.pdf}\\
    \includegraphics[]{figure/selfsup_robotcar/img_1.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/hybrid_1.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/vitb_1.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/monodepth2_1.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/packnet-sfm_1.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/rmsfm_1.pdf}\\
    \includegraphics[]{figure/selfsup_robotcar/img_2.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/hybrid_2.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/vitb_2.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/monodepth2_2.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/packnet-sfm_2.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/rmsfm_2.pdf}\\
    \includegraphics[]{figure/selfsup_robotcar/img_3.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/hybrid_3.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/vitb_3.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/monodepth2_3.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/packnet-sfm_3.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/rmsfm_3.pdf}\\
    \includegraphics[]{figure/selfsup_robotcar/img_4.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/hybrid_4.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/vitb_4.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/monodepth2_4.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/packnet-sfm_4.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/rmsfm_4.pdf}\\
    \includegraphics[]{figure/selfsup_robotcar/img_5.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/hybrid_5.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/vitb_5.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/monodepth2_5.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/packnet-sfm_5.pdf}&
    \includegraphics[]{figure/selfsup_robotcar/rmsfm_5.pdf}\\

     \fontsize{120}{50} \selectfont Input images & \fontsize{120}{50} \selectfont Ours-Hybrid & 
     \fontsize{120}{50} \selectfont Ours-ViT&
     \fontsize{120}{50} \selectfont Monodepth2& \fontsize{120}{50} \selectfont PackNet-SfM&
     \fontsize{120}{50} \selectfont R-MSFM6
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\label{figure_result_kitti}
\end{figure*}

\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccc}
    \includegraphics[]{figure/sup_robotcar/img_0.pdf}&
    \includegraphics[]{figure/sup_robotcar/bts_0.pdf}&
    \includegraphics[]{figure/sup_robotcar/adabins_0.pdf}&
    \includegraphics[]{figure/sup_robotcar/transdepth_0.pdf}&
    \includegraphics[]{figure/sup_robotcar/depthformer_0.pdf}&
    \includegraphics[]{figure/sup_robotcar/glpdepth_0.pdf}\\
    \includegraphics[]{figure/sup_robotcar/img_1.pdf}&
    \includegraphics[]{figure/sup_robotcar/bts_1.pdf}&
    \includegraphics[]{figure/sup_robotcar/adabins_1.pdf}&
    \includegraphics[]{figure/sup_robotcar/transdepth_1.pdf}&
    \includegraphics[]{figure/sup_robotcar/depthformer_1.pdf}&
    \includegraphics[]{figure/sup_robotcar/glpdepth_1.pdf}\\
    \includegraphics[]{figure/sup_robotcar/img_2.pdf}&
    \includegraphics[]{figure/sup_robotcar/bts_2.pdf}&
    \includegraphics[]{figure/sup_robotcar/adabins_2.pdf}&
    \includegraphics[]{figure/sup_robotcar/transdepth_2.pdf}&
    \includegraphics[]{figure/sup_robotcar/depthformer_2.pdf}&
    \includegraphics[]{figure/sup_robotcar/glpdepth_2.pdf}\\
    \includegraphics[]{figure/sup_robotcar/img_3.pdf}&
    \includegraphics[]{figure/sup_robotcar/bts_3.pdf}&
    \includegraphics[]{figure/sup_robotcar/adabins_3.pdf}&
    \includegraphics[]{figure/sup_robotcar/transdepth_3.pdf}&
    \includegraphics[]{figure/sup_robotcar/depthformer_3.pdf}&
    \includegraphics[]{figure/sup_robotcar/glpdepth_3.pdf}\\
    \includegraphics[]{figure/sup_robotcar/img_4.pdf}&
    \includegraphics[]{figure/sup_robotcar/bts_4.pdf}&
    \includegraphics[]{figure/sup_robotcar/adabins_4.pdf}&
    \includegraphics[]{figure/sup_robotcar/transdepth_4.pdf}&
    \includegraphics[]{figure/sup_robotcar/depthformer_4.pdf}&
    \includegraphics[]{figure/sup_robotcar/glpdepth_4.pdf}\\
    \includegraphics[]{figure/sup_robotcar/img_5.pdf}&
    \includegraphics[]{figure/sup_robotcar/bts_5.pdf}&
    \includegraphics[]{figure/sup_robotcar/adabins_5.pdf}&
    \includegraphics[]{figure/sup_robotcar/transdepth_5.pdf}&
    \includegraphics[]{figure/sup_robotcar/depthformer_5.pdf}&
    \includegraphics[]{figure/sup_robotcar/glpdepth_5.pdf}\\

     \fontsize{120}{50} \selectfont Input images & \fontsize{120}{50} \selectfont BTS & 
     \fontsize{120}{50} \selectfont AdaBins&
     \fontsize{120}{50} \selectfont TransDepth& \fontsize{120}{50} \selectfont DepthForemr&
     \fontsize{120}{50} \selectfont GLPDepth
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\label{figure_result_kitti}
\end{figure*}

\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cccccc}
    \includegraphics[]{figure/sup_raincs/img_0.pdf}&
    \includegraphics[]{figure/sup_raincs/bts_0.pdf}&
    \includegraphics[]{figure/sup_raincs/adabins_0.pdf}&
    \includegraphics[]{figure/sup_raincs/transdepth_0.pdf}&
    \includegraphics[]{figure/sup_raincs/depthformer_0.pdf}&
    \includegraphics[]{figure/sup_raincs/glpdepth_0.pdf}\\
    \includegraphics[]{figure/sup_raincs/img_1.pdf}&
    \includegraphics[]{figure/sup_raincs/bts_1.pdf}&
    \includegraphics[]{figure/sup_raincs/adabins_1.pdf}&
    \includegraphics[]{figure/sup_raincs/transdepth_1.pdf}&
    \includegraphics[]{figure/sup_raincs/depthformer_1.pdf}&
    \includegraphics[]{figure/sup_raincs/glpdepth_1.pdf}\\
    \includegraphics[]{figure/sup_raincs/img_2.pdf}&
    \includegraphics[]{figure/sup_raincs/bts_2.pdf}&
    \includegraphics[]{figure/sup_raincs/adabins_2.pdf}&
    \includegraphics[]{figure/sup_raincs/transdepth_2.pdf}&
    \includegraphics[]{figure/sup_raincs/depthformer_2.pdf}&
    \includegraphics[]{figure/sup_raincs/glpdepth_2.pdf}\\
    \includegraphics[]{figure/sup_raincs/img_3.pdf}&
    \includegraphics[]{figure/sup_raincs/bts_3.pdf}&
    \includegraphics[]{figure/sup_raincs/adabins_3.pdf}&
    \includegraphics[]{figure/sup_raincs/transdepth_3.pdf}&
    \includegraphics[]{figure/sup_raincs/depthformer_3.pdf}&
    \includegraphics[]{figure/sup_raincs/glpdepth_3.pdf}\\
    \includegraphics[]{figure/sup_raincs/img_4.pdf}&
    \includegraphics[]{figure/sup_raincs/bts_4.pdf}&
    \includegraphics[]{figure/sup_raincs/adabins_4.pdf}&
    \includegraphics[]{figure/sup_raincs/transdepth_4.pdf}&
    \includegraphics[]{figure/sup_raincs/depthformer_4.pdf}&
    \includegraphics[]{figure/sup_raincs/glpdepth_4.pdf}\\

     \fontsize{120}{50} \selectfont Input images & \fontsize{120}{50} \selectfont BTS & 
     \fontsize{120}{50} \selectfont AdaBins&
     \fontsize{120}{50} \selectfont TransDepth& \fontsize{120}{50} \selectfont DepthForemr&
     \fontsize{120}{50} \selectfont GLPDepth
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\label{figure_result_kitti}
\end{figure*}


\begin{figure*}[t]
     \newcommand\w{10cm}
    \newcommand\h{5cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccc}
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_0.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_1.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_2.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_3.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_4.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_5.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_6.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_7.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_8.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_9.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_10.pdf}\\ 
        
     \fontsize{40}{40} \selectfont Input images & 
     \fontsize{40}{40} \selectfont GT depths &
     \fontsize{40}{40} \selectfont Hybrid &
     \fontsize{40}{40} \selectfont ViT &
     \fontsize{40}{40} \selectfont ConvNeXt & 
     \fontsize{40}{40} \selectfont SLaK & 
     \fontsize{40}{40} \selectfont RegionViT&
     \fontsize{40}{40} \selectfont Twins
     
     
    \end{tabular}}
    \caption{\textbf{Comparison of depth map results on various dataset.} We test our model and the competitive models trained on KITTI using MVS, SUN3D, RGBD, Scenes11 (Top to Bottom).}
    \label{figure_result_demons}
     \end{figure*}

\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccc}
     \includegraphics[]{figure/formers_pencil/img_0.pdf}& 
     \includegraphics[]{figure/formers_pencil/convnext_0.pdf}&  
     \includegraphics[]{figure/formers_pencil/SLaK_0.pdf}&  
     \includegraphics[]{figure/formers_pencil/region_0.pdf}&  
     \includegraphics[]{figure/formers_pencil/twins_0.pdf}\\
     \includegraphics[]{figure/formers_pencil/img_1.pdf}& 
     \includegraphics[]{figure/formers_pencil/convnext_1.pdf}&  
     \includegraphics[]{figure/formers_pencil/SLaK_1.pdf}&  
     \includegraphics[]{figure/formers_pencil/region_1.pdf}&  
     \includegraphics[]{figure/formers_pencil/twins_1.pdf}\\
     \includegraphics[]{figure/formers_pencil/img_2.pdf}& 
     \includegraphics[]{figure/formers_pencil/convnext_2.pdf}&  
     \includegraphics[]{figure/formers_pencil/SLaK_2.pdf}&  
     \includegraphics[]{figure/formers_pencil/region_2.pdf}&  
     \includegraphics[]{figure/formers_pencil/twins_2.pdf}\\
     \includegraphics[]{figure/formers_pencil/img_3.pdf}& 
     \includegraphics[]{figure/formers_pencil/convnext_3.pdf}&  
     \includegraphics[]{figure/formers_pencil/SLaK_3.pdf}&  
     \includegraphics[]{figure/formers_pencil/region_3.pdf}&  
     \includegraphics[]{figure/formers_pencil/twins_3.pdf}\\
     \includegraphics[]{figure/formers_pencil/img_4.pdf}& 
     \includegraphics[]{figure/formers_pencil/convnext_4.pdf}&  
     \includegraphics[]{figure/formers_pencil/SLaK_4.pdf}&  
     \includegraphics[]{figure/formers_pencil/region_4.pdf}&  
     \includegraphics[]{figure/formers_pencil/twins_4.pdf}\\
     \includegraphics[]{figure/formers_pencil/img_5.pdf}& 
     \includegraphics[]{figure/formers_pencil/convnext_5.pdf}&  
     \includegraphics[]{figure/formers_pencil/SLaK_5.pdf}&  
     \includegraphics[]{figure/formers_pencil/region_5.pdf}&  
     \includegraphics[]{figure/formers_pencil/twins_5.pdf}\\
     \includegraphics[]{figure/formers_pencil/img_6.pdf}& 
     \includegraphics[]{figure/formers_pencil/convnext_6.pdf}&  
     \includegraphics[]{figure/formers_pencil/SLaK_6.pdf}&  
     \includegraphics[]{figure/formers_pencil/region_6.pdf}&  
     \includegraphics[]{figure/formers_pencil/twins_6.pdf}\\
      \includegraphics[]{figure/formers_pencil/img_7.pdf}& 
     \includegraphics[]{figure/formers_pencil/convnext_7.pdf}&  
     \includegraphics[]{figure/formers_pencil/SLaK_7.pdf}&  
     \includegraphics[]{figure/formers_pencil/region_7.pdf}&  
     \includegraphics[]{figure/formers_pencil/twins_7.pdf}\\
     \fontsize{120}{50} \selectfont Input images & 
     \fontsize{120}{50} \selectfont ConvNeXt & 
     \fontsize{120}{50} \selectfont SLaK&
     \fontsize{120}{50} \selectfont RegionViT& 
     \fontsize{120}{50} \selectfont Twins
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\end{figure*}

\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccc}
     \includegraphics[]{figure/formers_style/img_0.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_0.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_0.pdf}&  
     \includegraphics[]{figure/formers_style/region_0.pdf}&  
     \includegraphics[]{figure/formers_style/twins_0.pdf}\\
     \includegraphics[]{figure/formers_style/img_1.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_1.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_1.pdf}&  
     \includegraphics[]{figure/formers_style/region_1.pdf}&  
     \includegraphics[]{figure/formers_style/twins_1.pdf}\\
     \includegraphics[]{figure/formers_style/img_2.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_2.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_2.pdf}&  
     \includegraphics[]{figure/formers_style/region_2.pdf}&  
     \includegraphics[]{figure/formers_style/twins_2.pdf}\\
     \includegraphics[]{figure/formers_style/img_3.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_3.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_3.pdf}&  
     \includegraphics[]{figure/formers_style/region_3.pdf}&  
     \includegraphics[]{figure/formers_style/twins_3.pdf}\\
     \includegraphics[]{figure/formers_style/img_4.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_4.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_4.pdf}&  
     \includegraphics[]{figure/formers_style/region_4.pdf}&  
     \includegraphics[]{figure/formers_style/twins_4.pdf}\\
     \includegraphics[]{figure/formers_style/img_5.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_5.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_5.pdf}&  
     \includegraphics[]{figure/formers_style/region_5.pdf}&  
     \includegraphics[]{figure/formers_style/twins_5.pdf}\\
     \includegraphics[]{figure/formers_style/img_6.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_6.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_6.pdf}&  
     \includegraphics[]{figure/formers_style/region_6.pdf}&  
     \includegraphics[]{figure/formers_style/twins_6.pdf}\\
      \includegraphics[]{figure/formers_style/img_7.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_7.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_7.pdf}&  
     \includegraphics[]{figure/formers_style/region_7.pdf}&  
     \includegraphics[]{figure/formers_style/twins_7.pdf}\\
     \fontsize{120}{50} \selectfont Input images & 
     \fontsize{120}{50} \selectfont ConvNeXt & 
     \fontsize{120}{50} \selectfont SLaK&
     \fontsize{120}{50} \selectfont RegionViT& 
     \fontsize{120}{50} \selectfont Twins
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\end{figure*}

\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccc}
     \includegraphics[]{figure/formers_water/img_0.pdf}& 
     \includegraphics[]{figure/formers_water/convnext_0.pdf}&  
     \includegraphics[]{figure/formers_water/SLaK_0.pdf}&  
     \includegraphics[]{figure/formers_water/region_0.pdf}&  
     \includegraphics[]{figure/formers_water/twins_0.pdf}\\
     \includegraphics[]{figure/formers_water/img_1.pdf}& 
     \includegraphics[]{figure/formers_water/convnext_1.pdf}&  
     \includegraphics[]{figure/formers_water/SLaK_1.pdf}&  
     \includegraphics[]{figure/formers_water/region_1.pdf}&  
     \includegraphics[]{figure/formers_water/twins_1.pdf}\\
     \includegraphics[]{figure/formers_water/img_2.pdf}& 
     \includegraphics[]{figure/formers_water/convnext_2.pdf}&  
     \includegraphics[]{figure/formers_water/SLaK_2.pdf}&  
     \includegraphics[]{figure/formers_water/region_2.pdf}&  
     \includegraphics[]{figure/formers_water/twins_2.pdf}\\
     \includegraphics[]{figure/formers_water/img_3.pdf}& 
     \includegraphics[]{figure/formers_water/convnext_3.pdf}&  
     \includegraphics[]{figure/formers_water/SLaK_3.pdf}&  
     \includegraphics[]{figure/formers_water/region_3.pdf}&  
     \includegraphics[]{figure/formers_water/twins_3.pdf}\\
     \fontsize{120}{50} \selectfont Input images & 
     \fontsize{120}{50} \selectfont ConvNeXt & 
     \fontsize{120}{50} \selectfont SLaK&
     \fontsize{120}{50} \selectfont RegionViT& 
     \fontsize{120}{50} \selectfont Twins
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\end{figure*}

\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccccc}
    \includegraphics[]{figure/foggy_selfsup/img_0.pdf}&
    \includegraphics[]{figure/foggy_selfsup/gt1_0.pdf}&
    \includegraphics[]{figure/foggy_selfsup/hybrid_0.pdf}&
    \includegraphics[]{figure/foggy_selfsup/vitb_0.pdf}&
    \includegraphics[]{figure/foggy_selfsup/monodepth2_0.pdf}&
    \includegraphics[]{figure/foggy_selfsup/packnet-sfm_0.pdf}&
    \includegraphics[]{figure/foggy_selfsup/rmsfm_0.pdf}\\
    \includegraphics[]{figure/foggy_selfsup/img_1.pdf}&
    \includegraphics[]{figure/foggy_selfsup/gt1_1.pdf}&
    \includegraphics[]{figure/foggy_selfsup/hybrid_1.pdf}&
    \includegraphics[]{figure/foggy_selfsup/vitb_1.pdf}&
    \includegraphics[]{figure/foggy_selfsup/monodepth2_1.pdf}&
    \includegraphics[]{figure/foggy_selfsup/packnet-sfm_1.pdf}&
    \includegraphics[]{figure/foggy_selfsup/rmsfm_1.pdf}\\
    \includegraphics[]{figure/foggy_selfsup/img_2.pdf}&
    \includegraphics[]{figure/foggy_selfsup/gt1_2.pdf}&
    \includegraphics[]{figure/foggy_selfsup/hybrid_2.pdf}&
    \includegraphics[]{figure/foggy_selfsup/vitb_2.pdf}&
    \includegraphics[]{figure/foggy_selfsup/monodepth2_2.pdf}&
    \includegraphics[]{figure/foggy_selfsup/packnet-sfm_2.pdf}&
    \includegraphics[]{figure/foggy_selfsup/rmsfm_2.pdf}\\
    \includegraphics[]{figure/foggy_selfsup/img_3.pdf}&
    \includegraphics[]{figure/foggy_selfsup/gt1_3.pdf}&
    \includegraphics[]{figure/foggy_selfsup/hybrid_3.pdf}&
    \includegraphics[]{figure/foggy_selfsup/vitb_3.pdf}&
    \includegraphics[]{figure/foggy_selfsup/monodepth2_3.pdf}&
    \includegraphics[]{figure/foggy_selfsup/packnet-sfm_3.pdf}&
    \includegraphics[]{figure/foggy_selfsup/rmsfm_3.pdf}\\
    \includegraphics[]{figure/foggy_selfsup/img_4.pdf}&
    \includegraphics[]{figure/foggy_selfsup/gt1_4.pdf}&
    \includegraphics[]{figure/foggy_selfsup/hybrid_4.pdf}&
    \includegraphics[]{figure/foggy_selfsup/vitb_4.pdf}&
    \includegraphics[]{figure/foggy_selfsup/monodepth2_4.pdf}&
    \includegraphics[]{figure/foggy_selfsup/packnet-sfm_4.pdf}&
    \includegraphics[]{figure/foggy_selfsup/rmsfm_4.pdf}\\
    \includegraphics[]{figure/foggy_selfsup/img_5.pdf}&
    \includegraphics[]{figure/foggy_selfsup/gt1_5.pdf}&
    \includegraphics[]{figure/foggy_selfsup/hybrid_5.pdf}&
    \includegraphics[]{figure/foggy_selfsup/vitb_5.pdf}&
    \includegraphics[]{figure/foggy_selfsup/monodepth2_5.pdf}&
    \includegraphics[]{figure/foggy_selfsup/packnet-sfm_5.pdf}&
    \includegraphics[]{figure/foggy_selfsup/rmsfm_5.pdf}\\
    \includegraphics[]{figure/foggy_selfsup/img_6.pdf}&
    \includegraphics[]{figure/foggy_selfsup/gt1_6.pdf}&
    \includegraphics[]{figure/foggy_selfsup/hybrid_6.pdf}&
    \includegraphics[]{figure/foggy_selfsup/vitb_6.pdf}&
    \includegraphics[]{figure/foggy_selfsup/monodepth2_6.pdf}&
    \includegraphics[]{figure/foggy_selfsup/packnet-sfm_6.pdf}&
    \includegraphics[]{figure/foggy_selfsup/rmsfm_6.pdf}\\
    \includegraphics[]{figure/foggy_selfsup/img_7.pdf}&
    \includegraphics[]{figure/foggy_selfsup/gt1_7.pdf}&
    \includegraphics[]{figure/foggy_selfsup/hybrid_7.pdf}&
    \includegraphics[]{figure/foggy_selfsup/vitb_7.pdf}&
    \includegraphics[]{figure/foggy_selfsup/monodepth2_7.pdf}&
    \includegraphics[]{figure/foggy_selfsup/packnet-sfm_7.pdf}&
    \includegraphics[]{figure/foggy_selfsup/rmsfm_7.pdf}\\

     \fontsize{120}{50} \selectfont Input images &
     \fontsize{120}{50} \selectfont GT depths &
     \fontsize{120}{50} \selectfont Ours-Hybrid & 
     \fontsize{120}{50} \selectfont Ours-ViT&
     \fontsize{120}{50} \selectfont Monodepth2& 
     \fontsize{120}{50} \selectfont PackNet-SfM&
     \fontsize{120}{50} \selectfont R-MSFM6
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\label{figure_result_kitti}
\end{figure*}

\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccccc}
    \includegraphics[]{figure/foggy_sup/img_0.pdf}&
    \includegraphics[]{figure/foggy_sup/gt1_0.pdf}&
    \includegraphics[]{figure/foggy_sup/bts_0.pdf}&
    \includegraphics[]{figure/foggy_sup/adabins_0.pdf}&
    \includegraphics[]{figure/foggy_sup/transdepth_0.pdf}&
    \includegraphics[]{figure/foggy_sup/depthformer_0.pdf}&
    \includegraphics[]{figure/foggy_sup/glpdepth_0.pdf}\\
    \includegraphics[]{figure/foggy_sup/img_1.pdf}&
    \includegraphics[]{figure/foggy_sup/gt1_1.pdf}&
    \includegraphics[]{figure/foggy_sup/bts_1.pdf}&
    \includegraphics[]{figure/foggy_sup/adabins_1.pdf}&
    \includegraphics[]{figure/foggy_sup/transdepth_1.pdf}&
    \includegraphics[]{figure/foggy_sup/depthformer_1.pdf}&
    \includegraphics[]{figure/foggy_sup/glpdepth_1.pdf}\\
    \includegraphics[]{figure/foggy_sup/img_2.pdf}&
    \includegraphics[]{figure/foggy_sup/gt1_2.pdf}&
    \includegraphics[]{figure/foggy_sup/bts_2.pdf}&
    \includegraphics[]{figure/foggy_sup/adabins_2.pdf}&
    \includegraphics[]{figure/foggy_sup/transdepth_2.pdf}&
    \includegraphics[]{figure/foggy_sup/depthformer_2.pdf}&
    \includegraphics[]{figure/foggy_sup/glpdepth_2.pdf}\\
    \includegraphics[]{figure/foggy_sup/img_3.pdf}&
    \includegraphics[]{figure/foggy_sup/gt1_3.pdf}&
    \includegraphics[]{figure/foggy_sup/bts_3.pdf}&
    \includegraphics[]{figure/foggy_sup/adabins_3.pdf}&
    \includegraphics[]{figure/foggy_sup/transdepth_3.pdf}&
    \includegraphics[]{figure/foggy_sup/depthformer_3.pdf}&
    \includegraphics[]{figure/foggy_sup/glpdepth_3.pdf}\\
    \includegraphics[]{figure/foggy_sup/img_4.pdf}&
    \includegraphics[]{figure/foggy_sup/gt1_4.pdf}&
    \includegraphics[]{figure/foggy_sup/bts_4.pdf}&
    \includegraphics[]{figure/foggy_sup/adabins_4.pdf}&
    \includegraphics[]{figure/foggy_sup/transdepth_4.pdf}&
    \includegraphics[]{figure/foggy_sup/depthformer_4.pdf}&
    \includegraphics[]{figure/foggy_sup/glpdepth_4.pdf}\\
    \includegraphics[]{figure/foggy_sup/img_5.pdf}&
    \includegraphics[]{figure/foggy_sup/gt1_5.pdf}&
    \includegraphics[]{figure/foggy_sup/bts_5.pdf}&
    \includegraphics[]{figure/foggy_sup/adabins_5.pdf}&
    \includegraphics[]{figure/foggy_sup/transdepth_5.pdf}&
    \includegraphics[]{figure/foggy_sup/depthformer_5.pdf}&
    \includegraphics[]{figure/foggy_sup/glpdepth_5.pdf}\\
    \includegraphics[]{figure/foggy_sup/img_6.pdf}&
    \includegraphics[]{figure/foggy_sup/gt1_6.pdf}&
    \includegraphics[]{figure/foggy_sup/bts_6.pdf}&
    \includegraphics[]{figure/foggy_sup/adabins_6.pdf}&
    \includegraphics[]{figure/foggy_sup/transdepth_6.pdf}&
    \includegraphics[]{figure/foggy_sup/depthformer_6.pdf}&
    \includegraphics[]{figure/foggy_sup/glpdepth_6.pdf}\\
    \includegraphics[]{figure/foggy_sup/img_7.pdf}&
    \includegraphics[]{figure/foggy_sup/gt1_7.pdf}&
    \includegraphics[]{figure/foggy_sup/bts_7.pdf}&
    \includegraphics[]{figure/foggy_sup/adabins_7.pdf}&
    \includegraphics[]{figure/foggy_sup/transdepth_7.pdf}&
    \includegraphics[]{figure/foggy_sup/depthformer_7.pdf}&
    \includegraphics[]{figure/foggy_sup/glpdepth_7.pdf}\\
     \fontsize{120}{50} \selectfont Input images & 
     \fontsize{120}{50} \selectfont GT Depths & 
     \fontsize{120}{50} \selectfont BTS & 
     \fontsize{120}{50} \selectfont AdaBins&
     \fontsize{120}{50} \selectfont TransDepth& 
     \fontsize{120}{50} \selectfont DepthForemr&
     \fontsize{120}{50} \selectfont GLPDepth
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\label{figure_result_kitti}
\end{figure*}

\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccc}
     \includegraphics[]{figure/raincs_monoformers/img_0.pdf}& 
     \includegraphics[]{figure/raincs_monoformers/convnext_0.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/SLaK_0.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/region_0.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/twins_0.pdf}\\
     \includegraphics[]{figure/raincs_monoformers/img_1.pdf}& 
     \includegraphics[]{figure/raincs_monoformers/convnext_1.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/SLaK_1.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/region_1.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/twins_1.pdf}\\
     \includegraphics[]{figure/raincs_monoformers/img_2.pdf}& 
     \includegraphics[]{figure/raincs_monoformers/convnext_2.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/SLaK_2.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/region_2.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/twins_2.pdf}\\
     \includegraphics[]{figure/raincs_monoformers/img_3.pdf}& 
     \includegraphics[]{figure/raincs_monoformers/convnext_3.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/SLaK_3.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/region_3.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/twins_3.pdf}\\
     \includegraphics[]{figure/raincs_monoformers/img_4.pdf}& 
     \includegraphics[]{figure/raincs_monoformers/convnext_4.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/SLaK_4.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/region_4.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/twins_4.pdf}\\
     \fontsize{120}{50} \selectfont Input images & 
     \fontsize{120}{50} \selectfont ConvNeXt & 
     \fontsize{120}{50} \selectfont SLaK&
     \fontsize{120}{50} \selectfont RegionViT& 
     \fontsize{120}{50} \selectfont Twins
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\end{figure*}

\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccc}
     \includegraphics[]{figure/robotcar_monoformers/img_0.pdf}& 
     \includegraphics[]{figure/robotcar_monoformers/convnext_0.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/SLaK_0.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/region_0.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/twins_0.pdf}\\
     \includegraphics[]{figure/robotcar_monoformers/img_1.pdf}& 
     \includegraphics[]{figure/robotcar_monoformers/convnext_1.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/SLaK_1.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/region_1.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/twins_1.pdf}\\
     \includegraphics[]{figure/robotcar_monoformers/img_2.pdf}& 
     \includegraphics[]{figure/robotcar_monoformers/convnext_2.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/SLaK_2.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/region_2.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/twins_2.pdf}\\
     \includegraphics[]{figure/robotcar_monoformers/img_3.pdf}& 
     \includegraphics[]{figure/robotcar_monoformers/convnext_3.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/SLaK_3.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/region_3.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/twins_3.pdf}\\
     \includegraphics[]{figure/robotcar_monoformers/img_4.pdf}& 
     \includegraphics[]{figure/robotcar_monoformers/convnext_4.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/SLaK_4.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/region_4.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/twins_4.pdf}\\
     \fontsize{120}{50} \selectfont Input images & 
     \fontsize{120}{50} \selectfont ConvNeXt & 
     \fontsize{120}{50} \selectfont SLaK&
     \fontsize{120}{50} \selectfont RegionViT& 
     \fontsize{120}{50} \selectfont Twins
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\end{figure*}


\begin{figure*}[t]
     \newcommand\w{10cm}
    \newcommand\h{5cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccc}
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_0.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_1.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_2.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_3.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_4.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_5.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_6.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_7.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_8.pdf}\\ 

        
     \fontsize{40}{40} \selectfont Input images & 
     \fontsize{40}{40} \selectfont GT depths &
     \fontsize{40}{40} \selectfont Hybrid &
     \fontsize{40}{40} \selectfont ViT &
     \fontsize{40}{40} \selectfont ConvNeXt & 
     \fontsize{40}{40} \selectfont SLaK & 
     \fontsize{40}{40} \selectfont RegionViT&
     \fontsize{40}{40} \selectfont Twins
     
     
    \end{tabular}}
    \caption{\textbf{Comparison of depth map results on various dataset.} We test our model and the competitive models trained on KITTI using MVS, SUN3D, RGBD, Scenes11 (Top to Bottom).}
    \label{figure_result_demons}
     \end{figure*}

\begin{figure*}[t]
     \newcommand\w{10cm}
    \newcommand\h{5cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccc}
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_0.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_1.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_2.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_3.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_4.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_5.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_6.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_7.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_8.pdf}\\ 

        
     \fontsize{40}{40} \selectfont Input images & 
     \fontsize{40}{40} \selectfont GT depths &
     \fontsize{40}{40} \selectfont Hybrid &
     \fontsize{40}{40} \selectfont ViT &
     \fontsize{40}{40} \selectfont ConvNeXt & 
     \fontsize{40}{40} \selectfont SLaK & 
     \fontsize{40}{40} \selectfont RegionViT&
     \fontsize{40}{40} \selectfont Twins
     
     
    \end{tabular}}
    \caption{\textbf{Comparison of depth map results on various dataset.} We test our model and the competitive models trained on KITTI using MVS, SUN3D, RGBD, Scenes11 (Top to Bottom).}
    \label{figure_result_demons}
     \end{figure*}
     
     
\begin{figure*}[t]
     \newcommand\w{10cm}
    \newcommand\h{5cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_0.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_0.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_0.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_1.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_1.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_1.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_2.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_2.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_2.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_3.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_3.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_3.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_4.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_4.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_4.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_5.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_5.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_5.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_6.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_6.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_6.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_7.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_7.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_7.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_8.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_8.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_8.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_9.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_9.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_9.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_10.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_10.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_10.pdf}\\ 
        
     \fontsize{40}{40} \selectfont Input images & 
     \fontsize{40}{40} \selectfont GT depths &
    %  \fontsize{40}{40} \selectfont Hybrid &
    %  \fontsize{40}{40} \selectfont ViT &
     \fontsize{40}{40} \selectfont ConvNeXt & 
     \fontsize{40}{40} \selectfont SLaK & 
     \fontsize{40}{40} \selectfont RegionViT&
     \fontsize{40}{40} \selectfont Twins
     
     
    \end{tabular}}
    \caption{\textbf{Comparison of depth map results on various dataset.} We test our model and the competitive models trained on KITTI using MVS, SUN3D, RGBD, Scenes11 (Top to Bottom).}
    \label{figure_result_demons}
     \end{figure*}

\begin{figure*}[t]
     \newcommand\w{10cm}
    \newcommand\h{5cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_0.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_1.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_2.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_3.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_4.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_5.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_6.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_7.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_8.pdf}\\ 

        
     \fontsize{40}{40} \selectfont Input images & 
     \fontsize{40}{40} \selectfont GT depths &
     \fontsize{40}{40} \selectfont ConvNeXt & 
     \fontsize{40}{40} \selectfont SLaK & 
     \fontsize{40}{40} \selectfont RegionViT&
     \fontsize{40}{40} \selectfont Twins
     
     
    \end{tabular}}
    \caption{\textbf{Comparison of depth map results on various dataset.} We test our model and the competitive models trained on KITTI using MVS, SUN3D, RGBD, Scenes11 (Top to Bottom).}
    \label{figure_result_demons}
     \end{figure*}
     
     \begin{figure*}[t]
     \newcommand\w{10cm}
    \newcommand\h{5cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_0.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_1.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_2.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_3.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_4.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_5.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_6.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_7.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_8.pdf}\\ 

        
     \fontsize{40}{40} \selectfont Input images & 
     \fontsize{40}{40} \selectfont GT depths &
     \fontsize{40}{40} \selectfont ConvNeXt & 
     \fontsize{40}{40} \selectfont SLaK & 
     \fontsize{40}{40} \selectfont RegionViT&
     \fontsize{40}{40} \selectfont Twins
     
     
    \end{tabular}}
    \caption{\textbf{Comparison of depth map results on various dataset.} We test our model and the competitive models trained on KITTI using MVS, SUN3D, RGBD, Scenes11 (Top to Bottom).}
    \label{figure_result_demons}
     \end{figure*}

\end{fig}

==> no_insert_figure.tex <==

%selfsup-rain
    % \includegraphics[]{figure/selfsup_raincs/img_0.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/hybrid_0.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/vitb_0.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/monodepth2_0.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/packnet-sfm_0.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/rmsfm_0.pdf}\\
    % \includegraphics[]{figure/selfsup_raincs/img_4.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/hybrid_4.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/vitb_4.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/monodepth2_4.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/packnet-sfm_4.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/rmsfm_4.pdf}\\
    % \includegraphics[]{figure/selfsup_raincs/img_5.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/hybrid_5.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/vitb_5.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/monodepth2_5.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/packnet-sfm_5.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/rmsfm_5.pdf}\\
    % \includegraphics[]{figure/selfsup_raincs/img_6.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/hybrid_6.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/vitb_6.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/monodepth2_6.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/packnet-sfm_6.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/rmsfm_6.pdf}\\
    % \includegraphics[]{figure/selfsup_raincs/img_3.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/hybrid_3.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/vitb_3.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/monodepth2_3.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/packnet-sfm_3.pdf}&
    % \includegraphics[]{figure/selfsup_raincs/rmsfm_3.pdf}\\
    
%selfsup-night
    % \includegraphics[]{figure/selfsup_robotcar/img_3.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/hybrid_3.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/vitb_3.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/monodepth2_3.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/packnet-sfm_3.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/rmsfm_3.pdf}\\
    % \includegraphics[]{figure/selfsup_robotcar/img_4.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/hybrid_4.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/vitb_4.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/monodepth2_4.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/packnet-sfm_4.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/rmsfm_4.pdf}\\
    % \includegraphics[]{figure/selfsup_robotcar/img_0.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/hybrid_0.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/vitb_0.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/monodepth2_0.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/packnet-sfm_0.pdf}&
    % \includegraphics[]{figure/selfsup_robotcar/rmsfm_0.pdf}\\
    
%selfsup-foggy
    % \includegraphics[]{figure/foggy_selfsup/img_0.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/gt1_0.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/hybrid_0.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/vitb_0.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/monodepth2_0.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/packnet-sfm_0.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/rmsfm_0.pdf}\\
    % \includegraphics[]{figure/foggy_selfsup/img_1.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/gt1_1.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/hybrid_1.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/vitb_1.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/monodepth2_1.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/packnet-sfm_1.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/rmsfm_1.pdf}\\
    % \includegraphics[]{figure/foggy_selfsup/img_2.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/gt1_2.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/hybrid_2.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/vitb_2.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/monodepth2_2.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/packnet-sfm_2.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/rmsfm_2.pdf}\\
    % \includegraphics[]{figure/foggy_selfsup/img_3.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/gt1_3.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/hybrid_3.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/vitb_3.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/monodepth2_3.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/packnet-sfm_3.pdf}&
    % \includegraphics[]{figure/foggy_selfsup/rmsfm_3.pdf}\\
    
%sup-demons
        % \includegraphics[width=\w,height=\h]{figure/sup_demon/img_rgbd_0170.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/sup_demon/gt_rgbd_0170.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/sup_demon/BTS_rgbd_0170.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/sup_demon/Adabins_rgbd_0170.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/sup_demon/Transdepth_rgbd_0170.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/sup_demon/Depthformer_rgbd_0170.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/sup_demon/GLPDepth_rgbd_0170.pdf}\\
        % \includegraphics[width=\w,height=\h]{figure/sup_demon/img_scenes11_0391.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/sup_demon/gt_scenes11_0391.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/sup_demon/BTS_scenes11_0391.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/sup_demon/Adabins_scenes11_0391.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/sup_demon/Transdepth_scenes11_0391.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/sup_demon/Depthformer_scenes11_0391.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/sup_demon/GLPDepth_scenes11_0391.pdf}\\ 
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/img_courtyard_0000.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_courtyard_0000.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_courtyard_0000.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_courtyard_0000.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_courtyard_0000.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_courtyard_0000.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_courtyard_0000.pdf}\\
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/img_courtyard_0013.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_courtyard_0013.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_courtyard_0013.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_courtyard_0013.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_courtyard_0013.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_courtyard_0013.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_courtyard_0013.pdf}\\
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/img_delivery_area_0008.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_delivery_area_0008.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_delivery_area_0008.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_delivery_area_0008.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_delivery_area_0008.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_delivery_area_0008.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_delivery_area_0008.pdf}\\
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/img_facade_0002.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_facade_0002.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_facade_0002.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_facade_0002.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_facade_0002.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_facade_0002.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_facade_0002.pdf}\\
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/img_kicker_0008.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_kicker_0008.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_kicker_0008.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_kicker_0008.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_kicker_0008.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_kicker_0008.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_kicker_0008.pdf}\\
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/img_kicker_0026.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_kicker_0026.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_kicker_0026.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_kicker_0026.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_kicker_0026.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_kicker_0026.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_kicker_0026.pdf}\\
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/img_pipes_0004.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_pipes_0004.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_pipes_0004.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_pipes_0004.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_pipes_0004.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_pipes_0004.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_pipes_0004.pdf}\\
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/img_pipes_0007.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/gt_pipes_0007.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/BTS_pipes_0007.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Adabins_pipes_0007.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Transdepth_pipes_0007.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/Depthformer_pipes_0007.pdf}&
        % \includegraphics[width=\w,height=\h]{figure/sup_eth/GLPDepth_pipes_0007.pdf}\\

%sup-artifical
    % \includegraphics[]{figure/sup_kitti/img_KITTI_water_1.pdf}& 
    % \includegraphics[]{figure/sup_kitti/KITTI_water_BTS_1.pdf}&  
    % \includegraphics[]{figure/sup_kitti/KITTI_water_Adabins_1.pdf}&
    % \includegraphics[]{figure/sup_kitti/KITTI_water_Transdepth_1.pdf}&
    % \includegraphics[]{figure/sup_kitti/KITTI_water_Depthformer_1.pdf}&
    % \includegraphics[]{figure/sup_kitti/KITTI_water_GLPDepth_1.pdf}\\
    
    % \includegraphics[]{figure/sup_kitti/img_KITTI_style1_7.pdf}& 
    % \includegraphics[]{figure/sup_kitti/KITTI_style1_BTS_7.pdf}&  
    % \includegraphics[]{figure/sup_kitti/KITTI_style1_Adabins_7.pdf}&
    % \includegraphics[]{figure/sup_kitti/KITTI_style1_Transdepth_7.pdf}&
    % \includegraphics[]{figure/sup_kitti/KITTI_style1_Depthformer_7.pdf}&
    % \includegraphics[]{figure/sup_kitti/KITTI_style1_GLPDepth_7.pdf}\\
    

%sup-night
    % \includegraphics[]{figure/sup_robotcar/img_1.pdf}&
    % \includegraphics[]{figure/sup_robotcar/bts_1.pdf}&
    % \includegraphics[]{figure/sup_robotcar/adabins_1.pdf}&
    % \includegraphics[]{figure/sup_robotcar/transdepth_1.pdf}&
    % \includegraphics[]{figure/sup_robotcar/depthformer_1.pdf}&
    % \includegraphics[]{figure/sup_robotcar/glpdepth_1.pdf}\\
    % \includegraphics[]{figure/sup_robotcar/img_2.pdf}&
    % \includegraphics[]{figure/sup_robotcar/bts_2.pdf}&
    % \includegraphics[]{figure/sup_robotcar/adabins_2.pdf}&
    % \includegraphics[]{figure/sup_robotcar/transdepth_2.pdf}&
    % \includegraphics[]{figure/sup_robotcar/depthformer_2.pdf}&
    % \includegraphics[]{figure/sup_robotcar/glpdepth_2.pdf}\\
    %     \includegraphics[]{figure/sup_robotcar/img_5.pdf}&
    % \includegraphics[]{figure/sup_robotcar/bts_5.pdf}&
    % \includegraphics[]{figure/sup_robotcar/adabins_5.pdf}&
    % \includegraphics[]{figure/sup_robotcar/transdepth_5.pdf}&
    % \includegraphics[]{figure/sup_robotcar/depthformer_5.pdf}&
    % \includegraphics[]{figure/sup_robotcar/glpdepth_5.pdf}\\
    
%sup-rain
    % \includegraphics[]{figure/sup_raincs/img_2.pdf}&
    % \includegraphics[]{figure/sup_raincs/bts_2.pdf}&
    % \includegraphics[]{figure/sup_raincs/adabins_2.pdf}&
    % \includegraphics[]{figure/sup_raincs/transdepth_2.pdf}&
    % \includegraphics[]{figure/sup_raincs/depthformer_2.pdf}&
    % \includegraphics[]{figure/sup_raincs/glpdepth_2.pdf}\\
    % \includegraphics[]{figure/sup_raincs/img_4.pdf}&
    % \includegraphics[]{figure/sup_raincs/bts_4.pdf}&
    % \includegraphics[]{figure/sup_raincs/adabins_4.pdf}&
    % \includegraphics[]{figure/sup_raincs/transdepth_4.pdf}&
    % \includegraphics[]{figure/sup_raincs/depthformer_4.pdf}&
    % \includegraphics[]{figure/sup_raincs/glpdepth_4.pdf}\\
    
%sup-foggy
    % \includegraphics[]{figure/foggy_sup/img_1.pdf}&
    % \includegraphics[]{figure/foggy_sup/gt1_1.pdf}&
    % \includegraphics[]{figure/foggy_sup/bts_1.pdf}&
    % \includegraphics[]{figure/foggy_sup/adabins_1.pdf}&
    % \includegraphics[]{figure/foggy_sup/transdepth_1.pdf}&
    % \includegraphics[]{figure/foggy_sup/depthformer_1.pdf}&
    % \includegraphics[]{figure/foggy_sup/glpdepth_1.pdf}\\

    % \includegraphics[]{figure/foggy_sup/img_3.pdf}&
    % \includegraphics[]{figure/foggy_sup/gt1_3.pdf}&
    % \includegraphics[]{figure/foggy_sup/bts_3.pdf}&
    % \includegraphics[]{figure/foggy_sup/adabins_3.pdf}&
    % \includegraphics[]{figure/foggy_sup/transdepth_3.pdf}&
    % \includegraphics[]{figure/foggy_sup/depthformer_3.pdf}&
    % \includegraphics[]{figure/foggy_sup/glpdepth_3.pdf}\\

    % \includegraphics[]{figure/foggy_sup/img_5.pdf}&
    % \includegraphics[]{figure/foggy_sup/gt1_5.pdf}&
    % \includegraphics[]{figure/foggy_sup/bts_5.pdf}&
    % \includegraphics[]{figure/foggy_sup/adabins_5.pdf}&
    % \includegraphics[]{figure/foggy_sup/transdepth_5.pdf}&
    % \includegraphics[]{figure/foggy_sup/depthformer_5.pdf}&
    % \includegraphics[]{figure/foggy_sup/glpdepth_5.pdf}\\
    % \includegraphics[]{figure/foggy_sup/img_6.pdf}&
    % \includegraphics[]{figure/foggy_sup/gt1_6.pdf}&
    % \includegraphics[]{figure/foggy_sup/bts_6.pdf}&
    % \includegraphics[]{figure/foggy_sup/adabins_6.pdf}&
    % \includegraphics[]{figure/foggy_sup/transdepth_6.pdf}&
    % \includegraphics[]{figure/foggy_sup/depthformer_6.pdf}&
    % \includegraphics[]{figure/foggy_sup/glpdepth_6.pdf}\\
    
    
ours-all
\begin{figure*}[t]
     \newcommand\w{10cm}
    \newcommand\h{5cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccc}
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_0.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_1.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_2.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_3.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_4.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_5.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_6.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_7.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_8.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_9.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_10.pdf}\\ 
        
     \fontsize{40}{40} \selectfont Input images & 
     \fontsize{40}{40} \selectfont GT depths &
     \fontsize{40}{40} \selectfont Hybrid &
     \fontsize{40}{40} \selectfont ViT &
     \fontsize{40}{40} \selectfont ConvNeXt & 
     \fontsize{40}{40} \selectfont SLaK & 
     \fontsize{40}{40} \selectfont RegionViT&
     \fontsize{40}{40} \selectfont Twins
     
     
    \end{tabular}}
    \caption{\textbf{Comparison of depth map results on various dataset.} We test our model and the competitive models trained on KITTI using MVS, SUN3D, RGBD, Scenes11 (Top to Bottom).}
    \label{figure_result_demons}
     \end{figure*}


modern-artifical
\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccc}

     \includegraphics[]{figure/formers_pencil/img_1.pdf}& 
     \includegraphics[]{figure/formers_pencil/convnext_1.pdf}&  
     \includegraphics[]{figure/formers_pencil/SLaK_1.pdf}&  
     \includegraphics[]{figure/formers_pencil/region_1.pdf}&  
     \includegraphics[]{figure/formers_pencil/twins_1.pdf}\\
     \includegraphics[]{figure/formers_pencil/img_2.pdf}& 
     \includegraphics[]{figure/formers_pencil/convnext_2.pdf}&  
     \includegraphics[]{figure/formers_pencil/SLaK_2.pdf}&  
     \includegraphics[]{figure/formers_pencil/region_2.pdf}&  
     \includegraphics[]{figure/formers_pencil/twins_2.pdf}\\
     \includegraphics[]{figure/formers_pencil/img_4.pdf}& 
     \includegraphics[]{figure/formers_pencil/convnext_4.pdf}&  
     \includegraphics[]{figure/formers_pencil/SLaK_4.pdf}&  
     \includegraphics[]{figure/formers_pencil/region_4.pdf}&  
     \includegraphics[]{figure/formers_pencil/twins_4.pdf}\\
     \includegraphics[]{figure/formers_pencil/img_5.pdf}& 
     \includegraphics[]{figure/formers_pencil/convnext_5.pdf}&  
     \includegraphics[]{figure/formers_pencil/SLaK_5.pdf}&  
     \includegraphics[]{figure/formers_pencil/region_5.pdf}&  
     \includegraphics[]{figure/formers_pencil/twins_5.pdf}\\
     \includegraphics[]{figure/formers_pencil/img_6.pdf}& 
     \includegraphics[]{figure/formers_pencil/convnext_6.pdf}&  
     \includegraphics[]{figure/formers_pencil/SLaK_6.pdf}&  
     \includegraphics[]{figure/formers_pencil/region_6.pdf}&  
     \includegraphics[]{figure/formers_pencil/twins_6.pdf}\\
      \includegraphics[]{figure/formers_pencil/img_7.pdf}& 
     \includegraphics[]{figure/formers_pencil/convnext_7.pdf}&  
     \includegraphics[]{figure/formers_pencil/SLaK_7.pdf}&  
     \includegraphics[]{figure/formers_pencil/region_7.pdf}&  
     \includegraphics[]{figure/formers_pencil/twins_7.pdf}\\
     \fontsize{120}{50} \selectfont Input images & 
     \fontsize{120}{50} \selectfont ConvNeXt & 
     \fontsize{120}{50} \selectfont SLaK&
     \fontsize{120}{50} \selectfont RegionViT& 
     \fontsize{120}{50} \selectfont Twins
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\end{figure*}


\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccc}
     \includegraphics[]{figure/formers_style/img_0.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_0.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_0.pdf}&  
     \includegraphics[]{figure/formers_style/region_0.pdf}&  
     \includegraphics[]{figure/formers_style/twins_0.pdf}\\
     \includegraphics[]{figure/formers_style/img_1.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_1.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_1.pdf}&  
     \includegraphics[]{figure/formers_style/region_1.pdf}&  
     \includegraphics[]{figure/formers_style/twins_1.pdf}\\
     \includegraphics[]{figure/formers_style/img_2.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_2.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_2.pdf}&  
     \includegraphics[]{figure/formers_style/region_2.pdf}&  
     \includegraphics[]{figure/formers_style/twins_2.pdf}\\
     \includegraphics[]{figure/formers_style/img_3.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_3.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_3.pdf}&  
     \includegraphics[]{figure/formers_style/region_3.pdf}&  
     \includegraphics[]{figure/formers_style/twins_3.pdf}\\
     \includegraphics[]{figure/formers_style/img_4.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_4.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_4.pdf}&  
     \includegraphics[]{figure/formers_style/region_4.pdf}&  
     \includegraphics[]{figure/formers_style/twins_4.pdf}\\
     \includegraphics[]{figure/formers_style/img_5.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_5.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_5.pdf}&  
     \includegraphics[]{figure/formers_style/region_5.pdf}&  
     \includegraphics[]{figure/formers_style/twins_5.pdf}\\
      \includegraphics[]{figure/formers_style/img_7.pdf}& 
     \includegraphics[]{figure/formers_style/convnext_7.pdf}&  
     \includegraphics[]{figure/formers_style/SLaK_7.pdf}&  
     \includegraphics[]{figure/formers_style/region_7.pdf}&  
     \includegraphics[]{figure/formers_style/twins_7.pdf}\\
     \fontsize{120}{50} \selectfont Input images & 
     \fontsize{120}{50} \selectfont ConvNeXt & 
     \fontsize{120}{50} \selectfont SLaK&
     \fontsize{120}{50} \selectfont RegionViT& 
     \fontsize{120}{50} \selectfont Twins
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\end{figure*}

\begin{figure*}[t!] 
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccc}

     \includegraphics[]{figure/formers_water/img_1.pdf}& 
     \includegraphics[]{figure/formers_water/convnext_1.pdf}&  
     \includegraphics[]{figure/formers_water/SLaK_1.pdf}&  
     \includegraphics[]{figure/formers_water/region_1.pdf}&  
     \includegraphics[]{figure/formers_water/twins_1.pdf}\\
     \includegraphics[]{figure/formers_water/img_2.pdf}& 
     \includegraphics[]{figure/formers_water/convnext_2.pdf}&  
     \includegraphics[]{figure/formers_water/SLaK_2.pdf}&  
     \includegraphics[]{figure/formers_water/region_2.pdf}&  
     \includegraphics[]{figure/formers_water/twins_2.pdf}\\

     \fontsize{120}{50} \selectfont Input images & 
     \fontsize{120}{50} \selectfont ConvNeXt & 
     \fontsize{120}{50} \selectfont SLaK&
     \fontsize{120}{50} \selectfont RegionViT& 
     \fontsize{120}{50} \selectfont Twins
    \end{tabular}}
    \caption{\textbf{Qualitative comparison to state-of-the-arts.} We use KITTI for training and testing.}
\end{figure*}


modern -rain
     \includegraphics[]{figure/raincs_monoformers/img_0.pdf}& 
     \includegraphics[]{figure/raincs_monoformers/convnext_0.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/SLaK_0.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/region_0.pdf}&  
     \includegraphics[]{figure/raincs_monoformers/twins_0.pdf}\\
     
    
modern-night
     \includegraphics[]{figure/robotcar_monoformers/img_0.pdf}& 
     \includegraphics[]{figure/robotcar_monoformers/convnext_0.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/SLaK_0.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/region_0.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/twins_0.pdf}\\
          \includegraphics[]{figure/robotcar_monoformers/img_2.pdf}& 
     \includegraphics[]{figure/robotcar_monoformers/convnext_2.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/SLaK_2.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/region_2.pdf}&  
     \includegraphics[]{figure/robotcar_monoformers/twins_2.pdf}\\
     

modenr-ethd-all
\begin{figure*}[t]
     \newcommand\w{10cm}
    \newcommand\h{5cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccc}
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_0.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_1.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_2.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_3.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_4.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_5.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_6.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_7.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/hybrid_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/vitb_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_8.pdf}\\ 

        
     \fontsize{40}{40} \selectfont Input images & 
     \fontsize{40}{40} \selectfont GT depths &
     \fontsize{40}{40} \selectfont Hybrid &
     \fontsize{40}{40} \selectfont ViT &
     \fontsize{40}{40} \selectfont ConvNeXt & 
     \fontsize{40}{40} \selectfont SLaK & 
     \fontsize{40}{40} \selectfont RegionViT&
     \fontsize{40}{40} \selectfont Twins
     
     
    \end{tabular}}
    \caption{\textbf{Comparison of depth map results on various dataset.} We test our model and the competitive models trained on KITTI using MVS, SUN3D, RGBD, Scenes11 (Top to Bottom).}
    \label{figure_result_demons}
     \end{figure*}
    
modern-foggy
\begin{figure*}[t]
     \newcommand\w{10cm}
    \newcommand\h{5cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_0.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_0.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_0.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_1.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_1.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_1.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_2.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_2.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_2.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_3.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_3.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_3.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_4.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_4.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_4.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_5.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_5.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_5.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_6.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_6.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_6.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_7.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_7.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_7.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_8.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_8.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_8.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_9.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_9.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_9.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_9.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/img_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/gt1_10.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/hybrid_10.pdf}& 
        % \includegraphics[width=\w,height=\h]{figure/formers_foggy/vitb_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/convnext_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/SLaK_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/region_10.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/formers_foggy/twins_10.pdf}\\ 
        
     \fontsize{40}{40} \selectfont Input images & 
     \fontsize{40}{40} \selectfont GT depths &
    %  \fontsize{40}{40} \selectfont Hybrid &
    %  \fontsize{40}{40} \selectfont ViT &
     \fontsize{40}{40} \selectfont ConvNeXt & 
     \fontsize{40}{40} \selectfont SLaK & 
     \fontsize{40}{40} \selectfont RegionViT&
     \fontsize{40}{40} \selectfont Twins
     
     
    \end{tabular}}
    \caption{\textbf{Comparison of depth map results on various dataset.} We test our model and the competitive models trained on KITTI using MVS, SUN3D, RGBD, Scenes11 (Top to Bottom).}
    \label{figure_result_demons}
     \end{figure*}

modern- diverse domain
\begin{figure*}[t]
     \newcommand\w{10cm}
    \newcommand\h{5cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccc}
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_0.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_1.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_2.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_3.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_4.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_5.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_6.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_7.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/hybrid_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/vitb_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_8.pdf}\\ 

        
     \fontsize{40}{40} \selectfont Input images & 
     \fontsize{40}{40} \selectfont GT depths &
     \fontsize{40}{40} \selectfont Hybrid &
     \fontsize{40}{40} \selectfont ViT &
     \fontsize{40}{40} \selectfont ConvNeXt & 
     \fontsize{40}{40} \selectfont SLaK & 
     \fontsize{40}{40} \selectfont RegionViT&
     \fontsize{40}{40} \selectfont Twins
     
     
    \end{tabular}}
    \caption{\textbf{Comparison of depth map results on various dataset.} We test our model and the competitive models trained on KITTI using MVS, SUN3D, RGBD, Scenes11 (Top to Bottom).}
    \label{figure_result_demons}
     \end{figure*}


modern-demon
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_1.pdf}\\ 
                \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_3.pdf}\\ 
                \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_2.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_6.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_7.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/img_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/gt1_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/convnext_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/SLaK_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/region_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/demon_monoformers/twins_8.pdf}\\ 
\begin{figure*}[t]
     \newcommand\w{10cm}
    \newcommand\h{5cm}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_0.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_0.pdf}\\
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_1.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_1.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_2.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_2.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_3.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_3.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_4.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_4.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_5.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_5.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_6.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_6.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_7.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_7.pdf}\\ 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/img_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/gt1_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/convnext_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/SLaK_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/region_8.pdf}& 
        \includegraphics[width=\w,height=\h]{figure/eth3d_monoformers/twins_8.pdf}\\ 

        
     \fontsize{40}{40} \selectfont Input images & 
     \fontsize{40}{40} \selectfont GT depths &
     \fontsize{40}{40} \selectfont ConvNeXt & 
     \fontsize{40}{40} \selectfont SLaK & 
     \fontsize{40}{40} \selectfont RegionViT&
     \fontsize{40}{40} \selectfont Twins
     
     
    \end{tabular}}
    \caption{\textbf{Comparison of depth map results on various dataset.} We test our model and the competitive models trained on KITTI using MVS, SUN3D, RGBD, Scenes11 (Top to Bottom).}
    \label{figure_result_demons}
     \end{figure*}

==> tab.tex <==
\begin{tab}

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline
\multirow{2}{*}{Model} & \multirow{2}{*}{Backbone} & \multicolumn{4}{c}{Lower is better \downarrow}                               & \multicolumn{3}{c}{Higher is better \uparrow}                               \\ \cline{3-9} 
                       &                           & Abs Rel        & Sq Rel         & RMSE           & RMSElog        & $\delta <1.25$  & $\delta < 1.25^2$ & $\delta < 1.25^3$ \\ \hline
BTS              & CNN                       & 0.061          & 0.250          & 2.803          & 0.098          & 0.954          & 0.992                   & 0.998                   \\
AdaBins             & CNN                       & 0.058          & 0.190          & 2.360          & 0.088          & 0.965          & 0.995                   & \textbf{0.999}                   \\ \hline
TransDepth            & CNN-Transformer                       & 0.064          & 0.252 & 2.755          & 0.098          & 0.956          & 0.994                   & \textbf{0.999}          \\
DepthFormer                & CNN-Transformer                       & \textbf{0.052}          & \textbf{0.156}          & \textbf{2.133}          & \textbf{0.079}          & \textbf{0.974}          & \textbf{0.997}                   & \textbf{0.999}                   \\ \hline
GLPDepth                & Transformer                       & 0.059          & 0.187          & \textbf{2.133}          & \textbf{0.079}          & \textbf{0.974}          & \textbf{0.997}                   & \textbf{0.999}                   \\ \hline

\end{tabular}%
}
\caption{\textbf{Quantitative results of state-of-the-arts about KITTI.} We are not retrain the models. We use the pretrained models that given by authors. This table is just for comparison of each models.}
    \label{table_resutl_kitti}
\end{table}


\begin{table}[t!]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccccccc}
\hline $\text{D}^*$ & Model & Abs Rel \downarrow & Sq Rel \downarrow & RMSE \downarrow &RMSElog \downarrow & $\delta < 1.25$ \uparrow & $\delta < 1.25^2$ \uparrow & $\delta < 1.25^3$ \uparrow \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{Water-color}}  & BTS       & 0.225          & 2.469          & 8.503          & 0.441          & 0.599	& 0.753 &	0.844         \\
                              & AdaBins          & 0.301&	2.938&	8.761&	0.525         & 0.415&	0.642&	0.782          \\ \cline{2-9}
                              & TransDepth          & 0.111	&0.728	&4.886&	0.179     & 0.855	&0.955&	0.985          \\ 
                              & DepthFormer       & 0.135 &	1.102&	5.983&	0.249 & 0.783&	0.905&	0.955 \\ \cline{2-9} 
                              & GLPDepth & \textbf{0.099}&	\textbf{0.573}&	\textbf{4.121}&	\textbf{0.165}& \textbf{0.872}&	\textbf{0.960}&\textbf{0.986}       \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{Pencil-sketch}} & BTS       & 0.247&	2.180&	7.956	&0.413          & 0.509	&0.745&	0.871         \\
                              & AdaBins          & 0.165&	1.133&	5.812&	0.262        &0.721&	0.889&	0.957          \\ \cline{2-9}
                              & TransDepth          &0.136	&0.987	&5.774	&0.221          & 0.775 &	0.926&	0.975          \\ 
                              & DepthFormer       &0.162&	1.290&	6.498&	0.272 & 0.713&	0.885	&0.953  \\ \cline{2-9} 
                              & GLPDepth & \textbf{0.992}&	\textbf{0.513}&	\textbf{3.950}	&\textbf{0.157} & \textbf{0.874}&\textbf{0.970}&\textbf{0.992}  \\ \hline       
\multirow{5}{*}{\rotatebox[origin=c]{90}{Style-transfer}}  
                              &BTS       & 0.284	&3.233&	9.300&	0.550         & 0.512&	0.674&	0.770         \\
                              & AdaBins          & 0.317	&3.500&	9.594&	0.579       &0.414&	0.626&	0.751        \\ \cline{2-9}
                              & TransDepth          &0.146&	1.127&	5.910&	0.238         & 0.761&	0.911&	0.964          \\ 
                              & DepthFormer       &0.274&	2.766&	8.366&	0.493 & 0.501&	0.691&	0.801 \\ \cline{2-9} 
                              & GLPDepth & \textbf{0.099}&	\textbf{0.513}&\textbf{3.950}&	\textbf{0.157} & \textbf{0.874}&\textbf{0.970}&\textbf{0.992}  \\ \hline 
\end{tabular}}
\caption{\textbf{Quantitative comparison on texture-shifted datasets.} $\text{D}^*$ is datasets.}
\label{table_result_texture}
\vspace{-0.4cm}
\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccccc}
\hline
$\text{D}^*$ & Model & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ & $\delta < 1.25 \uparrow$ & $\delta < 1.25^2 \uparrow$ & $\delta < 1.25^3 \uparrow$ \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{MVS}} 
& BTS & 0.530 & 0.280 & 0.333 & 0.343 & 0.635 & 0.825 \\
 & AdaBins & 0.409 & 0.157 & 0.246 & 0.392 & 0.689 & 0.870 \\
 & TransDepth & 0.416 & 0.191 & 0.280 & 0.440 & 0.714 & 0.860 \\
 & DepthFormer & 0.369 & 0.158 & 0.259 & 0.516 & 0.793 & 0.906 \\
 & GLPDepth & \textbf{0.279} & \textbf{0.075} & \textbf{0.195} & \textbf{0.551} & \textbf{0.839} & \textbf{0.948} \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{RGBD}} 
& BTS & 0.551 & 0.197 & 0.293 & 0.278 & 0.504 & 0.695 \\
 & AdaBins & 0.448 & 0.126 & 0.261 & 0.269 & 0.539 & 0.760 \\
 & TransDepth & 0.416 & 0.138 & 0.237 & 0.409 & 0.663 & 0.826 \\
 & DepthFormer & 0.465 & 0.164 & 0.260 & 0.358 & 0.614 & 0.789 \\
 & GLPDepth & \textbf{0.381} & \textbf{0.111} & \textbf{0.225} & \textbf{0.442} & \textbf{0.680} & \textbf{0.837} \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{Scenes11}} 
& BTS & 2.446 & 0.844 & 0.269 & 0.269 & 0.496 & 0.663 \\
 & AdaBins & 2.583 & 0.992 & 0.265 & 0.277 & 0.512 & 0.675 \\
 & TransDepth & 1.830 & 0.464 & 0.233 & 0.313 & 0.565 & 0.723 \\
 & DepthFormer & 2.470 & 0.930 & 0.251 & 0.324 & 0.560 & 0.708 \\
 & GLPDepth & \textbf{1.811} & \textbf{0.439} & \textbf{0.226} & \textbf{0.391} & \textbf{0.625} & \textbf{0.757} \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{SUN3D}} 
& BTS & 0.403 & 0.145 & 0.268 & 0.380 & 0.664 & 0.842 \\
 & AdaBins & 0.353 & 0.112 & 0.240 & 0.400 & 0.683 & 0.854 \\
 & TransDepth & 0.297 & 0.087 & 0.218 & 0.511 & 0.793 & 0.908 \\
 & DepthFormer & 0.277 & 0.083 & \textbf{0.204} & \textbf{0.563} & \textbf{0.836} & \textbf{0.935} \\
 & GLPDepth & \textbf{0.273} & \textbf{0.074} & 0.207 & 0.533 & 0.819 & 0.928 \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{ETH3D}} 
&BTS&0.508&0.199&0.287&0.324&0.582&0.758\\
&Adabins&0.478&0.152&0.256&0.300&0.571&0.758\\
&Transdepth&0.370&0.108&0.220&0.427&0.696&0.846\\
&DepthFormer&\textbf{0.285}&0.079&\textbf{0.182}&0.573&\textbf{0.816}&\textbf{0.921}\\
&GLPdepth&0.290&\textbf{0.071}&0.191&\textbf{0.519}&0.786&0.905\\ \hline
\end{tabular}%
}
\caption{\textbf{Comparison results.} Evaluation of KITTI-trained model on diverse public datasets. $\text{D}^*$ is datasets.}
\vspace{-0.3cm}
\label{table_result_domains}
\end{table}

\begin{table*}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline $\text{D}^*$ & Backbone & Abs Rel \downarrow & Sq Rel \downarrow & RMSE \downarrow &RMSElog \downarrow & $\delta < 1.25$ \uparrow & $\delta < 1.25^2$ \uparrow & $\delta < 1.25^3$ \uparrow \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{{{\fontsize{8}{8} \selectfont Water-color}}}} 
& ConvNeXt & \textbf{0.159} & \textbf{1.175} & \textbf{5.971} & \textbf{0.244} & \textbf{0.774} & \textbf{0.921} & \textbf{0.969} \\
 & SLaK & 0.170 & 1.272 & 6.316 & 0.259 & 0.755 & 0.907 & 0.961 \\
 & RegionViT & 0.179 & 1.341 & 6.309 & 0.273 & 0.732 & 0.902 & 0.958 \\
 & Twins & 0.166 & 1.295 & 6.558 & 0.258 & 0.751 & 0.911 & 0.963 \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{{\fontsize{8}{8} \selectfont Pencil-sketch}}} 
& ConvNeXt & \textbf{0.176} & \textbf{1.280} & \textbf{6.582} & \textbf{0.262} & \textbf{0.728} & \textbf{0.907} & \textbf{0.965} \\
 & SLaK & 0.268 & 2.268 & 8.042 & 0.364 & 0.553 & 0.811 & 0.915 \\
 & RegionViT & 0.260 & 2.012 & 7.491 & 0.341 & 0.545 & 0.832 & 0.939 \\
 & Twins & 0.205 & 1.630 & 7.512 & 0.301 & 0.655 & 0.871 & 0.949 \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{{\fontsize{8}{8} \selectfont Style-transfer}}} 
& ConvNeXt & \textbf{0.219} & \textbf{1.722} & \textbf{7.214} & \textbf{0.315} & \textbf{0.634} & \textbf{0.861} &\textbf{0.942} \\
 & SLaK & 0.224 & 1.859 & 7.423 & 0.324 & 0.648 & 0.855 & 0.934 \\
 & RegionViT & 0.242 & 2.030 & 7.944 & 0.347 & 0.587 & 0.835 & 0.927 \\
 & Twins & 0.232 & 1.974 & 8.045 & 0.337 & 0.599 & 0.839 & 0.931 \\ \hline
\end{tabular}%
}
\caption{\textbf{Quantitative comparison on texture-shifted datasets.} $\text{D}^*$ is datasets.}
\end{table*}

\begin{table*}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline
$\text{D}^*$ & Backbone & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ & $\delta < 1.25 \uparrow$ & $\delta < 1.25^2 \uparrow$ & $\delta < 1.25^3 \uparrow$ \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{MVS}} 
& ConvNeXt & 0.259 & 0.060 & \textbf{0.171} & \textbf{0.582} & \textbf{0.863} & 0.949 \\
 & SLaK & 0.424 & 0.149 & 0.264 & 0.375 & 0.651 & 0.820 \\
 & RegionViT & 0.376 & 0.124 & 0.238 & 0.436 & 0.714 & 0.863 \\
 & Twins & \textbf{0.247} & \textbf{0.056} & \textbf{0.171} & 0.590 & 0.861 & \textbf{0.952} \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{RGBD}} 
& ConvNeXt & 0.346 & 0.094 & 0.208 & 0.438 & 0.706 & 0.860 \\
 & SLaK & 0.481 & 0.198 & 0.272 & 0.349 & 0.607 & 0.770 \\
 & RegionViT & 0.484 & 0.225 & 0.276 & 0.369 & 0.626 & 0.791 \\
 & Twins & \textbf{0.323} & \textbf{0.085} & \textbf{0.194} & \textbf{0.522} & \textbf{0.749} & \textbf{0.876} \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{Scenes11}} 
& ConvNeXt & 1.827 & 0.620 & 0.251 & 0.350 & 0.576 & 0.718 \\
 & SLaK & 1.913 & 0.533 & 0.263 & 0.295 & 0.525 & 0.680 \\
 & RegionViT & 1.866 & 0.486 & 0.257 & 0.316 & 0.546 & 0.695 \\
 & Twins & \textbf{1.503} & \textbf{0.316} & \textbf{0.233} & \textbf{0.387} & \textbf{0.615} & \textbf{0.749} \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{SUN3D}} 
& ConvNeXt & \textbf{0.254} & 0.061 & 0.182 & \textbf{0.538} & \textbf{0.833} & \textbf{0.942} \\
 & SLaK & 0.379 & 0.134 & 0.258 & 0.396 & 0.673 & 0.838 \\
 & RegionViT & 0.358 & 0.121 & 0.247 & 0.413 & 0.696 & 0.855 \\
 & Twins & 0.256 & \textbf{0.058} & \textbf{0.178} & 0.537 & 0.832 & 0.941 \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{ETH3D}} 
&ConvNeXt&0.271&0.063&\textbf{0.178}&\textbf{0.527}&\textbf{0.802}&0.920\\
&SLaK&0.386&0.115&0.226&0.375&0.652&0.821\\
&RegionViT&0.364&0.098&0.136&0.410&0.695&0.853\\
&Twins&\textbf{0.270}&\textbf{0.062}&0.182&0.531&0.801&\textbf{0.921}\\ \hline
\end{tabular}%
}
\end{table*}


\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
$\text{D}^*$ & Model & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ & $\delta < 1.25 \uparrow$ & $\delta < 1.25^2 \uparrow$ & $\delta < 1.25^3 \uparrow$ \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{MVS}} 
& Monodepth2 & 0.471 & 0.407 & 0.503 & 0.408 & 0.661 & 0.806 \\
 & PackNet-SfM & 0.449 & 0.295 & 0.429 & 0.397 & 0.670 & 0.837 \\
 & R-MSFM6 & 0.550 & 0.603 & 0.583 & 0.352 & 0.591 & 0.756 \\
 & Ours-ViT & 0.254 & 0.061 & 0.179 & 0.589 &0.865  & 0.952 \\
 & Ours-Hybrid & \textbf{0.231} & \textbf{0.052} & \textbf{0.167} & \textbf{0.617} & \textbf{0.883} & \textbf{0.960} \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{RGBD}} 
& Monodepth2 & 0.610 & 0.508 & 0.488 & 0.292 & 0.520 & 0.681 \\
 & PackNet-SfM & 0.593 & 0.416 & 0.460 & 0.318 & 0.562 & 0.731 \\
 & R-MSFM6 & 0.695 & 0.553 & 0.490 & 0.261 & 0.471 & 0.627 \\
 & Ours-ViT & 0.337 & 0.098 & 0.207 & 0.475 &0.747  & 0.874 \\
 & Ours-Hybrid & \textbf{0.302} & \textbf{0.085} & \textbf{0.193} & \textbf{0.532} & \textbf{0.766} & \textbf{0.888} \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{Scenes11}} 
& Monodepth2 & 1.647 & 0.763 & 0.356 & 0.312 & 0.529 & 0.671 \\
 & PackNet-SfM & 2.065 & 0.837 & 0.330 & 0.310 & 0.530 & 0.674 \\
 & R-MSFM6 & 1.727 & 0.726 & 0.361 & 0.280 & 0.494 & 0.636 \\
 & Ours-ViT & 1.476 & 0.314 & 0.219 & 0.419  & 0.657 & 0.776 \\
 & Ours-Hybrid & \textbf{1.220} & \textbf{0.213} & \textbf{0.214} & \textbf{0.433} & \textbf{0.667} & \textbf{0.780} \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{SUN3D}} 
& Monodepth2 & 0.554 & 0.535 & 0.576 & 0.324 & 0.556 & 0.718 \\
 & PackNet-SfM & 0.466 & 0.336 & 0.471 & 0.350 & 0.612 & 0.792 \\
 & R-MSFM6 & 0.523 & 0.406 & 0.506 & 0.310 & 0.544 & 0.721 \\
  & Ours-ViT & 0.244 & 0.059  & 0.1743 &0.570  & 0.844 & 0.946 \\
 & Ours-Hybrid & \textbf{0.232} & \textbf{0.051} & \textbf{0.167} & \textbf{0.586} & \textbf{0.860} & \textbf{0.953} \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{ETH3D}} 
&Monodepth2&0.449&0.219&0.267&0.397&0.629&0.753\\
&PackNet-SfM&0.359&0.119&0.218&0.436&0.700&0.839\\
&R-MSFM6&0.441&0.168&0.249&0.379&0.624&0.757\\
&Ours-ViT&0.249&0.056&0.167&0.559&0.826&0.933\\
&Ours-Hybrid&\textbf{0.232}&\textbf{0.050}&\textbf{0.160}&\textbf{0.587}&\textbf{0.851}&\textbf{0.946}\\ \hline
\end{tabular}}
\caption{\textbf{Comparison results.} Evaluation of KITTI-trained model on diverse public datasets. $\text{D}^*$ is datasets.}
\vspace{-0.3cm}
\label{table_result_domains}
\end{table}

\begin{table}[t!]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccccccc}
\hline $\text{D}^*$ & Model & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ &RMSElog $\downarrow$ & $\delta < 1.25$ $\uparrow$ & $\delta < 1.25^2 \uparrow$ & $\delta < 1.25^3 \uparrow$ \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{Water-color}}  & Monodepth2       & 0.170          & 1.345          & 6.175          & 0.263          & 0.750          & 0.909          & 0.960          \\
                              & PackNet-SfM          & 0.174          & 1.364          & 6.334          & 0.264          & 0.742          & 0.906          & 0.961          \\
                              & R-MSFM6          & 0.194          & 1.613          & 7.173          & 0.302          & 0.696          & 0.876          & 0.943          \\ \cline{2-9} 
                              & Ours-ViT       & 0.152          & 1.196          & 5.668          & 0.232 & 0.799 & 0.932 & 0.973 \\
                              & Ours-Hybrid & \textbf{0.140} & \textbf{1.053} & \textbf{5.665} & \textbf{0.222}          & \textbf{0.815}          & \textbf{0.936}          & \textbf{0.975}          \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{Pencil-sketch}} & Monodepth2       & 0.196          & 1.522          & 6.232          & 0.276          & 0.691          & 0.898          & 0.962          \\
                              & PackNet-SfM          & 0.204          & 1.569          & 6.568          & 0.290          & 0.670          & 0.888          & 0.957          \\
                              & R-MSFM6          & 0.217          & 1.698          & 6.719          & 0.301          & 0.647          & 0.872          & 0.951          \\ \cline{2-9} 
                              & Ours-ViT       & 0.174          & 1.311          & 5.770 & 0.248          & 0.756          & 0.920          & 0.967          \\
                              & Ours-Hybrid & \textbf{0.151} & \textbf{1.084} & \textbf{5.615}          & \textbf{0.227} & \textbf{0.786} & \textbf{0.934} & \textbf{0.976} \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{Style-transfer}}  & Monodepth2       &  0.247  &   2.440  &   7.525  &   0.343  &   0.617  &   0.828  &   0.920         \\
                              & PackNet-SfM          & 0.205   &  1.606   &  6.778   &  0.301   &  0.672   &  0.876   &  0.948\\
                              & R-MSFM6          &  0.294  &   2.788  &   8.579  &   0.396  &   0.521  &   0.770  &   0.894         \\ \cline{2-9} 
                              & Ours-ViT       &    0.186       &      1.379     &   6.652        &    0.274       & 0.705 & 0.898 &  0.959         \\
                              & Ours-Hybrid & \textbf{0.175} & \textbf{1.307} & \textbf{6.435} & \textbf{0.264} &   \textbf{0.728}        & \textbf{0.906} & \textbf{0.962} \\ \hline
\end{tabular}}
\caption{\textbf{Quantitative comparison on texture-shifted datasets.} $\text{D}^*$ is datasets.}
\label{table_result_texture}
\vspace{-0.4cm}
\end{table}



\begin{table}[t!]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccccccc}
\hline $\text{D}^*$ & Model & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ &RMSElog $\downarrow$ & $\delta < 1.25$ $\uparrow$ & $\delta < 1.25^2 \uparrow$ & $\delta < 1.25^3 \uparrow$ \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Oxford \\ RobotCar}}}  

& Monodepth2& 1.039&0.044&0.159&\textbf{0.113}&0.204&0.406&0.564\\
& PackNet-SfM & 1.080&0.045&0.159&0.114&0.193&0.378&0.536\\
& R-MSFM6 & 0.951&0.043&0.160&0.114&0.223&0.362&0.469	\\  \cline{2-9} 
& Ours-ViT&0.935&0.042&0.159&\textbf{0.113}&0.235&0.444&0.602	 \\
& Ours-Hybrid & \textbf{0.869}&\textbf{0.040}&\textbf{0.159}&\textbf{0.113}&\textbf{0.292}&\textbf{0.555}&\textbf{0.691}\\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Foggy \\ CityScapes}}} 
&Monodepth2&0.438&0.060&0.109&0.073&0.514&0.757&0.853 \\
&PackNet-SfM&0.457&0.055&0.102&0.070&0.545&0.782&0.873 \\
&R-MSFM6&0.435&0.062&0.124&0.080&0.442&0.697&0.809 \\ \cline{2-9}
&Ours-ViT&0.368&0.033&0.097&0.063&0.591&0.845&0.917 \\ 
&Ours-Hybrid&\textbf{0.316}&\textbf{0.025}&\textbf{0.080}&\textbf{0.053}&\textbf{0.674}&\textbf{0.879}&\textbf{0.929} \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Rainy \\ CityScapes}}}  
&Monodepth2&1.215&2.194&1.289&0.446&0.183&0.348&0.495 \\
&PackNet-SfM&1.151&1.771&1.169&0.410&0.234&0.444&0.609 \\
&R-MSFM6&1.310&3.028&1.509&0.495&0.171&0.315&0.441 \\ \cline{2-9}
&Ours-ViT&0.803&0.891&0.868&0.330&0.298&0.545&0.709 \\
&Ours-Hybrid&\textbf{0.788}&\textbf{0.707}&\textbf{0.752}&\textbf{0.297}&\textbf{0.323}&\textbf{0.574}&\textbf{0.738} \\ \hline
\end{tabular}}
\caption{\textbf{Quantitative comparison on texture-shifted datasets.} $\text{D}^*$ is datasets.}
\label{table_result_texture}
\vspace{-0.4cm}
\end{table}

\begin{table}[t!]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccccccc}
\hline $\text{D}^*$ & Model & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ &RMSElog $\downarrow$ & $\delta < 1.25$ $\uparrow$ & $\delta < 1.25^2 \uparrow$ & $\delta < 1.25^3 \uparrow$ \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Oxford \\ RobotCar}}}  
&BTS&0.707&0.039&0.160&0.114&0.340&0.604&0.723\\
&AdaBins&0.637&0.038&0.160&0.114&0.371&0.640&0.771\\\cline{2-9}
&TransDepth&0.531&\textbf{0.037}&\textbf{0.159}&\textbf{0.113}&0.430&0.645&0.768 \\ 
&DepthFormer&0.550&\textbf{0.037}&\textbf{0.159}&\textbf{0.113}&0.420&0.629&0.756 \\\cline{2-9}
&GLPDepth&\textbf{0.538}&\textbf{0.037}&\textbf{0.159}&\textbf{0.113}&\textbf{0.422}&\textbf{0.673}&\textbf{0.780} \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Foggy \\ CityScapes}}} 
&BTS&1.092&0.294&0.118&0.092&0.572&0.716&0.794 \\
&AdaBins&1.441&0.524&0.185&0.135&0.516&0.667&0.744 \\\cline{2-9}
&TransDepth&0.631&0.075&\textbf{0.069}&\textbf{0.055}&0.631&0.797&0.860\\ 
&DepthFormer&0.669&0.083&0.070&0.056&\textbf{0.636}&0.794&0.857\\\cline{2-9}
&GLPDepth&\textbf{0.594}&\textbf{0.070}&0.103&0.071&0.561&\textbf{0.799}&\textbf{0.872}\\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Rainy \\ CityScapes}}}  
&BTS&1.366&1.632&0.710&0.295&0.379&0.623&0.756\\
&AdaBins&1.299&1.452&0.668&0.267&0.330&0.585&0.771\\\cline{2-9}
&TransDepth&1.034&1.003&0.793&0.303&0.485&0.698&0.771\\ 
&DepthFormer&1.039&1.016&0.816&0.310&0.473&0.690&0.764\\\cline{2-9}
&GLPDepth&\textbf{1.030}&\textbf{0.928}&\textbf{0.560}&\textbf{0.258}&\textbf{0.513}&\textbf{0.742}&\textbf{0.822}\\ \hline
\end{tabular}}
\caption{\textbf{Quantitative comparison on texture-shifted datasets.} $\text{D}^*$ is datasets.}
\label{table_result_texture}
\vspace{-0.4cm}
\end{table}

\begin{table}[t!]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccccccc}
\hline $\text{D}^*$ & Model & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ &RMSElog $\downarrow$ & $\delta < 1.25$ $\uparrow$ & $\delta < 1.25^2 \uparrow$ & $\delta < 1.25^3 \uparrow$ \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Oxford \\ RobotCar}}}  
&ConvNeXt&\textbf{0.714}&\textbf{0.037}&\textbf{0.159}&\textbf{0.113}&\textbf{0.310}&\textbf{0.546}&\textbf{0.705}\\
&SLaK&0.916&0.041&0.160&0.114&0.210&0.425&0.594\\
&RegionViT&1.067&0.041&0.160&0.114&0.239&0.456&0.623\\
&Twins&0.831&0.037&\textbf{0.159}&\textbf{0.113}&0.300&0.516&0.686\\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Foggy \\ CityScapes}}} 
&ConvNeXt&0.353&0.031&0.090&0.058&0.638&\textbf{0.864}&\textbf{0.922}\\
&SLaK&0.839&0.151&0.205&0.141&0.209&0.440&0.652\\
&RegionViT&0.643&0.088&0.167&0.112&0.337&0.605&0.782\\
&Twins&\textbf{0.350}&\textbf{0.029}&\textbf{0.087}&\textbf{0.057}&\textbf{0.648}&0.862&0.920\\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Rainy \\ CityScapes}}}  
&ConvNeXt&\textbf{0.658}&\textbf{0.332}&\textbf{0.396}&\textbf{0.184}&\textbf{0.475}&\textbf{0.739}&\textbf{0.900}\\
&SLaK&0.856&0.510&0.460&0.220&0.356&0.631&0.822\\
&RegionViT&0.798&0.773&0.805&0.319&0.251&0.493&0.676\\
&Twins&0.795&0.825&0.829&0.322&0.285&0.526&0.688\\ \hline
\end{tabular}}
\caption{\textbf{Quantitative comparison on texture-shifted datasets.} $\text{D}^*$ is datasets.}
\label{table_result_texture}
\vspace{-0.4cm}
\end{table}

% \begin{table}[t!]
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{ccccccccc}
% \hline $\text{D}^*$ & Model & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ &RMSElog $\downarrow$ & $\delta < 1.25$ $\uparrow$ & $\delta < 1.25^2 \uparrow$ & $\delta < 1.25^3 \uparrow$ \\ \hline

% \multirow{14}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Oxford \\ RobotCar}}}  

% & Monodepth2& 1.039&0.044&0.159&0.113&0.204&0.406&0.564\\
% & PackNet-SfM & 1.080&0.045&0.159&0.114&0.193&0.378&0.536\\
% & R-MSFM6 & 0.951&0.043&0.160&0.114&0.223&0.362&0.469	\\  
% & Ours-ViT&0.935&0.042&0.159&0.113&0.235&0.444&0.602	 \\
% & Ours-Hybrid & 0.869&0.040&0.159&0.113&0.292&0.555&0.691\\ \cline{2-9} 

% &BTS&0.707&0.039&0.159&0.113&0.340&0.604&0.723\\
% &AdaBins&0.637&0.038&0.159&0.113&0.371&0.640&0.771\\\
% &TransDepth&0.531&0.037&0.159&0.113&0.430&0.645&0.768 \\ 
% &DepthFormer&0.550&0.037&0.159&0.113&0.420&0.629&0.756 \\
% &GLPDepth&0.538&0.037&0.159&0.113&0.422&0.673&0.780 \\ \cline{2-9} 

% &ConvNeXt&0.714&0.037&0.159&0.113&0.310&0.546&0.705\\
% &SLaK&0.916&0.041&0.159&0.113&0.210&0.425&0.594\\
% &RegionViT&1.067&0.041&0.159&0.113&0.239&0.456&0.623\\
% &Twins&0.831&0.037&0.159&0.113&0.300&0.516&0.686\\ \hline

% \multirow{14}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Foggy \\ CityScapes}}} 

% &Monodepth2&0.438&0.060&0.109&0.073&0.514&0.757&0.853 \\
% &PackNet-SfM&0.457&0.055&0.102&0.070&0.545&0.782&0.873 \\
% &R-MSFM6&0.435&0.062&0.124&0.080&0.442&0.697&0.809 \\
% &Ours-ViT&0.368&0.033&0.097&0.063&0.591&0.845&0.917 \\ 
% &Ours-Hybrid&0.316&0.025&0.080&0.053&0.674&0.879&0.929 \\ \cline{2-9}


% &BTS&1.092&0.294&0.118&0.092&0.572&0.716&0.794 \\
% &AdaBins&1.441&0.524&0.185&0.135&0.516&0.667&0.744 \\\
% &TransDepth&0.631&0.075&0.069&0.055&0.631&0.797&0.860\\ 
% &DepthFormer&0.669&0.083&0.070&0.056&0.636&0.794&0.857\\ 
% &GLPDepth&0.594&0.070&0.103&0.071&0.561&0.799&0.872\\ \cline{2-9} 

% &ConvNeXt&0.353&0.031&0.090&0.058&0.638&0.864&0.922\\
% &SLaK&0.839&0.151&0.205&0.141&0.209&0.440&0.652\\
% &RegionViT&0.643&0.088&0.167&0.112&0.337&0.605&0.782\\
% &Twins&0.350&0.029&0.087&0.057&0.648&0.862&0.920\\ \hline

% \multirow{14}{*}{\rotatebox[origin=c]{90}{\makecell[c]{Rainy \\ CityScapes}}}  

% &Monodepth2&1.215&2.194&1.289&0.446&0.183&0.348&0.495 \\
% &PackNet-SfM&1.151&1.771&1.169&0.410&0.234&0.444&0.609 \\
% &R-MSFM6&1.310&3.028&1.509&0.495&0.171&0.315&0.441 \\
% &Ours-ViT&0.803&0.891&0.868&0.330&0.298&0.545&0.709 \\
% &Ours-Hybrid&0.788&0.707&0.752&0.297&0.323&0.574&0.738 \\ \cline{2-9}


% &BTS&1.366&1.632&0.710&0.295&0.379&0.623&0.756\\
% &AdaBins&1.299&1.452&0.560&0.258&0.330&0.585&0.771\\
% &TransDepth&1.034&1.003&0.793&0.303&0.485&0.698&0.771\\ 
% &DepthFormer&1.039&1.016&0.816&0.310&0.473&0.690&0.764\\
% &GLPDepth&1.030&0.928&0.688&0.267&0.513&0.742&0.822\\  \cline{2-9} 

% &ConvNeXt&0.658&0.332&0.396&0.184&0.475&0.739&0.900\\
% &SLaK&0.856&0.510&0.460&0.220&0.356&0.631&0.822\\
% &RegionViT&0.798&0.773&0.805&0.319&0.251&0.493&0.676\\
% &Twins&0.795&0.825&0.829&0.322&0.285&0.526&0.688\\ \hline

% \end{tabular}}
% \caption{\textbf{Overview table of Practical texture-shifted datasets}}
% \label{table_result_texture}
% \vspace{-0.4cm}
% \end{table}




% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{ccccccccc}
% \hline $\text{D}^*$ & Backbone & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ & $\delta < 1.25 \uparrow$ & $\delta < 1.25^2 \uparrow$ & $\delta < 1.25^3 \uparrow$ \\ \hline
% % \multirow{14}{*}{\rotatebox[origin=c]{90}{MVS}} 
% % & Monodepth2 & 0.471 & 0.407 & 0.503 & 0.408 & 0.661 & 0.806 \\
% %  & PackNet-SfM & 0.449 & 0.295 & 0.429 & 0.397 & 0.670 & 0.837 \\
% %  & R-MSFM6 & 0.550 & 0.603 & 0.583 & 0.352 & 0.591 & 0.756 \\
% %  & Ours-ViT & 0.254 & 0.061 & 0.179 & 0.589 &0.865  & 0.952 \\
% %  & Ours-Hybrid & \textbf{0.231} & \textbf{0.052} & \textbf{0.167} & \textbf{0.617} & \textbf{0.883} & \textbf{0.960} \\ 

% % & ConvNeXt & 0.259 & 0.060 & 0.172 & 0.582 & 0.859 & 0.949 \\
% %  & SLaK & 0.424 & 0.149 & 0.264 & 0.375 & 0.651 & 0.820 \\
% %  & RegionViT & 0.376 & 0.124 & 0.238 & 0.436 & 0.714 & 0.863 \\
% %  & Twins & 0.247 & 0.056 & 0.171 & 0.590 & 0.861 & 0.952 \\ 

% %  & BTS & 0.530 & 0.280 & 0.333 & 0.343 & 0.635 & 0.825 \\
% %  & AdaBins & 0.409 & 0.157 & 0.246 & 0.392 & 0.689 & 0.870 \\
% %  & TransDepth & 0.416 & 0.191 & 0.280 & 0.440 & 0.714 & 0.860 \\
% %  & DepthFormer & 0.369 & 0.158 & 0.259 & 0.516 & 0.793 & 0.906 \\
% %  & GLPDepth & 0.279 & 0.075 & 0.195 & 0.551 & 0.839 & 0.948 \\ \hline

% % \multirow{14}{*}{\rotatebox[origin=c]{90}{RGBD}} 

% % & Monodepth2 & 0.610 & 0.508 & 0.488 & 0.292 & 0.520 & 0.681 \\
% %  & PackNet-SfM & 0.593 & 0.416 & 0.460 & 0.318 & 0.562 & 0.731 \\
% %  & R-MSFM6 & 0.695 & 0.553 & 0.490 & 0.261 & 0.471 & 0.627 \\
% %  & Ours-ViT & 0.337 & 0.098 & 0.207 & 0.475 &0.747  & 0.874 \\
% %  & Ours-Hybrid & \textbf{0.302} & \textbf{0.085} & \textbf{0.193} & \textbf{0.532} & \textbf{0.766} & \textbf{0.888} \\ 

% % & ConvNeXt & 0.346 & 0.094 & 0.208 & 0.438 & 0.706 & 0.860 \\
% %  & SLaK & 0.481 & 0.198 & 0.272 & 0.349 & 0.607 & 0.770 \\
% %  & RegionViT & 0.484 & 0.225 & 0.276 & 0.369 & 0.626 & 0.791 \\
% %  & Twins & 0.323 & 0.085 & 0.194 & 0.522 & 0.749 & 0.876 \\ 

% %  & BTS & 0.551 & 0.197 & 0.293 & 0.278 & 0.504 & 0.695 \\
% %  & AdaBins & 0.448 & 0.126 & 0.261 & 0.269 & 0.539 & 0.760 \\
% %  & TransDepth & 0.416 & 0.138 & 0.237 & 0.409 & 0.663 & 0.826 \\
% %  & DepthFormer & 0.465 & 0.164 & 0.260 & 0.358 & 0.614 & 0.789 \\
% %  & GLPDepth & 0.381 & 0.111 & 0.225 & 0.442 & 0.680 & 0.837 \\ \hline

% % \multirow{14}{*}{\rotatebox[origin=c]{90}{Scenes11}} 

% % & Monodepth2 & 1.647 & 0.763 & 0.356 & 0.312 & 0.529 & 0.671 \\
% %  & PackNet-SfM & 2.065 & 0.837 & 0.330 & 0.310 & 0.530 & 0.674 \\
% %  & R-MSFM6 & 1.727 & 0.726 & 0.361 & 0.280 & 0.494 & 0.636 \\
% %  & Ours-ViT & 1.476 & 0.314 & 0.219 & 0.419  & 0.657 & 0.776 \\
% %  & Ours-Hybrid & \textbf{1.220} & \textbf{0.213} & \textbf{0.214} & \textbf{0.433} & \textbf{0.667} & \textbf{0.780} \\ \hline

% % & ConvNeXt & 1.927 & 0.620 & 0.251 & 0.350 & 0.576 & 0.718 \\
% %  & SLaK & 1.913 & 0.533 & 0.263 & 0.295 & 0.525 & 0.680 \\
% %  & RegionViT & 1.866 & 0.486 & 0.257 & 0.316 & 0.546 & 0.695 \\
% %  & Twins & 1.503 & 0.316 & 0.233 & 0.387 & 0.615 & 0.749 \\ 

% %  & BTS & 2.446 & 0.844 & 0.269 & 0.269 & 0.496 & 0.663 \\
% %  & AdaBins & 2.583 & 0.992 & 0.265 & 0.277 & 0.512 & 0.675 \\
% %  & TransDepth & 1.830 & 0.464 & 0.233 & 0.313 & 0.565 & 0.723 \\
% %  & DepthFormer & 2.470 & 0.930 & 0.251 & 0.324 & 0.560 & 0.708 \\
% %  & GLPDepth & 1.811 & 0.439 & 0.226 & 0.391 & 0.625 & 0.757 \\ \hline

% % \multirow{14}{*}{\rotatebox[origin=c]{90}{SUN3D}} 
% % & Monodepth2 & 0.554 & 0.535 & 0.576 & 0.324 & 0.556 & 0.718 \\
% %  & PackNet-SfM & 0.466 & 0.336 & 0.471 & 0.350 & 0.612 & 0.792 \\
% %  & R-MSFM6 & 0.523 & 0.406 & 0.506 & 0.310 & 0.544 & 0.721 \\
% %   & Ours-ViT & 0.244 & 0.059  & 0.1743 &0.570  & 0.844 & 0.946 \\
% %  & Ours-Hybrid & \textbf{0.232} & \textbf{0.051} & \textbf{0.167} & \textbf{0.586} & \textbf{0.860} & \textbf{0.953} \\ 

% % & ConvNeXt & 0.254 & 0.061 & 0.182 & 0.538 & 0.833 & 0.942 \\
% %  & SLaK & 0.379 & 0.134 & 0.258 & 0.396 & 0.673 & 0.838 \\
% %  & RegionViT & 0.358 & 0.121 & 0.247 & 0.413 & 0.696 & 0.855 \\
% %  & Twins & 0.256 & 0.058 & 0.178 & 0.537 & 0.832 & 0.941 \\ 

% % & BTS & 0.403 & 0.145 & 0.268 & 0.380 & 0.664 & 0.842 \\
% %  & AdaBins & 0.353 & 0.112 & 0.240 & 0.400 & 0.683 & 0.854 \\
% %  & TransDepth & 0.297 & 0.087 & 0.218 & 0.511 & 0.793 & 0.908 \\
% %  & DepthFormer & 0.277 & 0.083 & 0.204 & 0.563 & 0.836 & 0.935 \\
% %  & GLPDepth & 0.273 & 0.074 & 0.207 & 0.533 & 0.819 & 0.928 \\ \hline

% \multirow{14}{*}{\rotatebox[origin=c]{90}{ETH3D}} 

% &Monodepth2&0.449&0.219&0.267&0.160&0.397&0.629&0.753\\
% &PackNet-SfM&0.359&0.119&0.218&0.138&0.436&0.700&0.839\\
% &R-MSFM6&0.441&0.168&0.249&0.157&0.379&0.624&0.757\\
% &Ours-ViT&0.249&0.056&0.167&0.106&0.559&0.826&0.933\\
% &Ours-Hybrid&0.232&0.050&0.160&0.101&0.587&0.851&0.946\\

% &ConvNeXt&0.271&0.063&0.178&0.113&0.527&0.802&0.920\\
% &SLaK&0.386&0.115&0.226&0.144&0.375&0.652&0.821\\
% &RegionViT&0.364&0.098&0.213&0.136&0.410&0.695&0.853\\
% &Twins&0.270&0.062&0.182&0.115&0.531&0.801&0.921\\ \hline

% &BTS&0.508&0.199&0.287&0.178&0.324&0.582&0.758\\
% &Adabins&0.478&0.152&0.256&0.167&0.300&0.571&0.758\\
% &Transdepth&0.370&0.108&0.220&0.141&0.427&0.696&0.846\\
% &DepthFormer&0.285&0.079&0.182&0.113&0.573&0.816&0.921\\
% &GLPdepth&0.290&0.071&0.191&0.121&0.519&0.786&0.905\\ \hline
% \end{tabular}%
% }
% \end{table*}



\begin{table}[t]
\begin{tabular}{cccccccc}
\hline
\multirow{2}{*}{Backbone} & \multicolumn{4}{c}{Lower is better \downarrow}             & \multicolumn{3}{c}{Higher is better \uparrow} \\ \cline{2-8} 
                          & Abs Rel & Sq Rel & RMSE & RMSElog & $\delta <1.25$     & $\delta < 1.25^2$     & $\delta < 1.25^3$     \\ \hline
ConvNeXt &  0.111   &  0.760   &  4.533   &  0.184   &  0.878   &  0.961   &  0.983   \\
SLaK &  0.117   &  0.866   &  4.811   &  0.199   &  0.866   &  0.947   &  0.976   \\
RegionViT &  0.113   &  0.893   &  4.756   &  0.193   &  0.875   &  0.954   &  0.979   \\
Twins &  0.125   &  1.309   &  4.973   &  0.197   &  0.866   &  0.948   &  0.974   \\ \hline
\end{tabular}
\end{table}

\begin{table}[t]
\begin{tabular}{cccccccc}
\hline
\multirow{2}{*}{Backbone} & \multicolumn{4}{c}{Lower is better \downarrow}             & \multicolumn{3}{c}{Higher is better \uparrow} \\ \cline{2-8} 
                          & Abs Rel & Sq Rel & RMSE & RMSElog & $\delta <1.25$     & $\delta < 1.25^2$     & $\delta < 1.25^3$     \\ \hline
ConvNeXt &  0.111   &  0.760   &  4.533   &  0.184   &  0.878   &  0.961   &  0.983   \\
SLaK &  0.117   &  0.866   &  4.811   &  0.199   &  0.866   &  0.947   &  0.976   \\
RegionViT &  0.113   &  0.893   &  4.756   &  0.193   &  0.875   &  0.954   &  0.979   \\
Twins &  0.125   &  1.309   &  4.973   &  0.197   &  0.866   &  0.948   &  0.974   \\ 
ViT &  0.117   &  0.884   &  4.783   &  0.193   &  0.869   &  0.956   &  0.981   \\
Hybrid & \textbf{0.104}   & \textbf{0.846}   &  \textbf{4.580}   &  \textbf{0.183}   &  \textbf{0.891}   &  \textbf{0.962}   &  \textbf{0.982}   \\ \hline
\end{tabular}
\end{table}

\end{tab}
